Performance-Aware Predictive-Model-Based On-Chip Body-Bias Regulation Strategy for an ULP Multi-Core Cluster in 28nm UTBB FD-SOI

The performance and reliability of Ultra-Low-Power (ULP) computing platforms are adversely affected by environmental temperature and process variations. Mitigating the effect of these phenomena becomes crucial when these devices operate near-threshold, due to the magnification of process variations and to the strong temperature inversion effect that affects advanced technology nodes in low-voltage corners, which causes huge overhead due to margining for timing closure. Supporting an extended range of reverse and forward body-bias, UTBB FD-SOI technology provides a powerful knob to compensate for such variations. In this work we propose a methodology to maximize energy efficiency at run-time exploiting body biasing on a ULP platform operating near-threshold. The proposed method relies on on-line performance measurements by means of Process Monitoring Blocks (PMBs) coupled with an on-chip low-power body bias generator. We correlate the measurement performed by the PMBs to the maximum achievable frequency of the system, deriving a predictive model able to estimate it with an error of 9.7% at 0.7V. To minimize the effect of process variations we propose a calibration procedure that allows to use a PMB model affected by only the temperature-induced error, which reduces the frequency estimation error by 2.4x (from 9.7% to 4%). We finally propose a controller architecture relying on the derived models to automatically regulate at run-time the body bias voltage. We demonstrate that adjusting the body bias voltage against environmental temperature variations leads up to 2X reduction in the leakage power and a 15% improvement on the global energy consumption when the system operates at 0.7V and 170MHz

==> Content/N0-1_relted_works.tex <==
\section{Related works}

Compensation of temperature-induced performance variations, as well as process variations is crucial in ULP application\cite{Alioto2012a}. In devices operating in near threshold, the dependency between temperature and device's frequency grows exponentially moving towards near threshold operating region. The issue of temperature compensation in CMOS devices has been extensively addressed several times, various studies propose solutions based on supply voltage adaptation\cite{Lee2014}\cite{Ono}. This has not been the case for the employment of body bias voltage to compensate temperature variation because different limiting factors\cite{Jacquet2014}\cite{Yeap2013}.
In bulk technologies, maximum body bias range is often limited by p-n junction leakage and potential latch up. In FinFET technologies, instead, the lack of an easy way to access the back gates represents the main obstacle.

%In most advanced CMOS technologies, thermal inversion causes an exponential growth of the dependency between temperature and frequency, especially when operating in near-threshold. Several works have addressed this problem, mainly leveraging adaptation of supply voltage \cite{Lee2014}\cite{Ono}. On the contrary, the adoption of body biasing to address variation of ambient temperature has not been extensively explored so far, due to the limited capabilities of most advanced technologies such as bulk and FinFET to provide extended body bias ranges suitable for compensation of wide temperature ranges \cite{Jacquet2014}\cite{Yeap2013}.

%both at the circuit level \cite{ONO_ESSCIRC_2004}, and at the architectural level \cite{BORTOLOTTI_PATMOS_2013}
%by a lack of advanced bulk planar technology (i.e., behind 28nm) , where the maximum body bias is limited by p-n junction leakage and potential latch-up, and FinFET technology missing an easy way to access the back gates . These technologies do not allow for temperature compensation through body biasing, and require the supply voltage to be adapted to match the frequency targets.
So far, the presented problems have been tackled by adopting conservative margins, both at design and run time, such as higher than necessary supply voltages or aggressive forward body biasing to cover all possible working scenarios. This highlight the fact that the mean used to compensate a performance gap is part of a broader issue, which is to make a system aware of its own maximum frequency and selectively modify run-time its parameter like body bias voltage to efficiently run at a target frequency. 

Different "on-line" performance estimation methodology have been proposed so far, however they are very often highly intrusive and rely on the deep knowledge of the system\cite{Blaauw_2008}. Methodologies based on Critical Path Replica (CPR) are a typical example\cite{Clerc2015}, but to implement such performance estimation, complete access to RTL is required. The reason why such methodology are not always applicable is that very often IPs composing a System on Chip (SoC) are provided as encripted macros or simply come as hardened macros from different design teams, so no access to RTL is possible. In the system we propose, a different performance monitoring solution is used: we embedded Performance Monitoring Blocks based on ring oscillator in each power domain of the system; this solution is completely architecture independent and does not require any knowledge of the RTL.

%Performance estimation methodologies can be used to automatize body-bias regulation in closed loop control structures. Our approach, differs from other approaches like \cite{Tschanz2007} since it relies on a direct frequency measurement instead of using look-up tables where the chip


%The methodologies proposed so far are very often highly intrusive and linked to a specific architecture. Solutions like the one proposed in \cite{Blaauw_2008} have to be fully integrated with the architecture to provide good results. Less intrusive solutions based on Critical Path Replicas (CPR) have been proposed \cite{Clerc2015}, but also in this case, the architecture's dependency of the performance monitoring system reduces the application field to designs where a complete access to all the SoC's IPs is possible. Contrary to what has been done so far, the performance monitoring system adopted in our solution keeps at minimum the intrusiveness, by exploiting on-chip direct frequency measurements. High generality is given by the fact that the knowledge of architectural details is not required, which is extremely useful when the IPs composing the system are released as encrypted macros, or simply come as hardened macros from different design teams.


==> Content/N00_abstract.tex <==
\begin{abstract}
Environmental temperature variations, as well as process variations, have a detrimental effect on performance and reliability of embedded systems implemented with deep-sub micron technologies. This sensitivity significantly increases in ultra-low-power (ULP) devices that operate in near-threshold, due to the magnification of process variations and to the strong thermal inversion that affects advanced technology nodes in low-voltage corner. Supporting an extended range of reverse and forward body-bias, UTBB FD-SOI technology provides a powerful knob to compensate for such variations.
In this work we propose a methodology to maximize, at run-time, the energy efficiency of the ultra-low-power systems exploiting body biasing. The proposed method relies on on-line performance measurements by means of Process Monitoring Blocks (PMBs) coupled with an on-chip low-power body bias generator. We characterize the response of the PMBs versus the maximum achievable frequency of the system, deriving a predictive model able to estimate such frequency with an error of 4\% at 0.7V.
We then propose a methodology considering forward body bias margins to minimize with a minimum cost the frequency estimation error.
We finally propose a controller architecture relying on the derived models to automatically regulate at run-time the body bias voltage. we find that adjusting the body bias voltage against environmental temperature variations leads upt to 2X reduction in the leakage power and a 1.3X improvement on the global power consumption when the system is operating at 0.7V and 160MHz.

%We apply this model to compensate Temperature-induced performance variations, estimating the maximum frequency with an error of 7\%; we eliminate the error by adding an appropriate body-bias margin resulting in a worst case global power consumption overhead of 5\%. As further improvement, we generalize the methodology to compensate also process variations, obtaining an error of 28\% on the estimated maximum performance and compensating this error with an overhead of 17\% on the global power consumption.

%correlating it with the operating frequency of the chip in a wide range of operating conditions obtaining three different levels of generality for the model:\textit{i)} Temperature/Process Independence achieving a worst-case accuracy of 72\% on the estimated frequency and an overhead in the power consumption of the 17\% \textit{ii)} Temperature Independence with a worst-case accuracy of 91\% and 5.5\% of overhead \textit{iii)} Operating Point dependence achieving an accuracy of 97 and an overhead of 3\%.

%and we correlated it with the model. The results of our exploration shows that leveraging body-biasing allows to compensate process variations and temperature variations in the range -20\textdegree C to 80\textdegree C with up to \hl{xx\%} energy saving with respect to compensation through adaptation of supply voltage only.

\end{abstract}

==> Content/N01_intro.tex <==
\section{Introduction}

%\IEEEPARstart{I}{nternet} of Things, e-Health, Smart Sensors and wearable consumer gadgets are expected to drive the electronic market of the next decades. These applications rely on the capability of the research community to provide devices that couple ultra-low power (ULP) behavior with a reasonable level of performance. Indeed, these applications are characterized not only by an increasingly tighter power budget, but also by an increasing demand of computation capabilities. The pace dictated by the Moore's law has slowed down, and CMOS scaling, which drove semiconductor growth during the past decades, is delivering reduced energy gains \cite{Dreslinski2010a}. In this “Moore's law twilight era”, further energy gain can be achieved by moving to the near-threshold computing (NTC) domain \cite{Markovic2010}. 
%However, electronic devices implemented with most advanced technological nodes feature a strong dependency between the ambient temperature and the operating frequency and leakage power. Unfortunately, this dependency increases in the near-threshold operating region, where ULP devices works to provide high energy efficiency \cite{Alioto2014}\cite{Pahlevan2016}\cite[p.~69]{Alioto2017}.

\IEEEPARstart{P}{ervasive} use of embedded computing platforms in e-Healt, wearable gadgets, smart sensors and Internet of things (IoT) applications is enforcing the research community to extensively explore the performance-energy solution's space. The need of more computationally capable devices is more and more often coupled with the limited power budget in which such platforms operate. IoT operating environment is giving rise to the establishment of Ultra-Low Power (ULP) devices, a new category of computing platforms designed to achieve very high energy efficiency in few milliwatt power envelopes.

Moore's Law, which perfectly described semiconductor growth during the past decades, has fulfilled its role. The huge effort required to develop latest scaled CMOS technological nodes is not delivering anymore the expected energy efficiency gains \cite{Dreslinski2010a}. Nowadays, a promising way is represented by the parallel near-threshold computing (NTC)\cite{Markovic2010}. The major challenge IoT devices have to face is operating in many different scenarios that are not always completely predictable at design time. more specifically, the main issue is constituted by different operating temperatures against a platform has to validated. This aspect is crucial, devices implemented in most advanced technological nodes have a strong dependency between environmental temperature and operating frequency and leakage power. \cite{Pahlevan2016}\cite{Alioto2017}. This behaviour is caused by a phenomenon called temperature effect inversion\cite{Lee2014}. In deep sub-micron technologies the detrimental effect that the temperature has on the maximum frequency of a device is reverted. More specifically, semiconductors' conductivity is governed by two concurrent factors: \textit{i)} carrier concentration which is positively affected by a temperature increase \textit{ii)} carriers mobility, which on the contrary degrades with a temperature increase. in most advanced technology, especially below 65nm, these two factors become more relevant\cite{Han2017}\cite{Pu2010}. Additionally, with the supply voltage lowering, the carrier concentration tends to affect more than carriers mobility the semiconductor conductivity. as a consequence, the performance of a device, as well as leakage current are positively affected by a temperature increase.
 
Another effect which must be taken into account in ULP devices implemented in recent technological nodes is process variation\footnote{We neglect the effect of aging since self-heating is minimum in ULP devices} which determines different performance of the chips depending on fluctuations of the manufacturing process. 
%The effects of process variations require a one-time compensation as soon as the chip is fabricated \footnote{Performance of digital circuits can also be affected by aging. However, since self-heating is minimal for systems operating in ULP domain, this phenomenon can be neglected.}. Contrarily, thermal variations are dependent on the operating environment, hence, they require a run-time compensation to ensure that chips are able to maximize the efficiency and at the same time guarantee a given target performance.
To align chips performance, post-silicon performance compensation can be achieved with different methodologies. Body biasing is a well known and reasonably easy to implement approach. with small transient current, it is possible to polarize the substrate of a device modifying its performance \cite{Sundaresan}\cite{Gammie2008}. Body biasing represents an alternative to adaptation of supply voltage, which requires more complex circuital solutions like on chip DC/DC converters or voltage regulators resulting in higher overheads.

The use of body biasing is twofold: \textit{i)} Forward Body Biasing (FBB) allows to increase the operating frequency of the chip with a minimum overhead on the dynamic power \textit{ii)} Reverse Body Biasing (RBB) can significantly reduce the leakage when the devices could run faster than target frequency because of process or operating conditions \cite{Rossi2015a}. 
%A well-known approach for achieving post-silicon tuning to compensate variations in circuits is through body biasing \cite{Tschanz2007}. As opposed to adaptation of supply voltage, that requires on chip DC/DC converters or voltage regulators, modulation of body biasing can be implemented with simpler and more efficient circuits, as relatively small transient currents are required to polarize the substrate of the devices \cite{Sundaresan} \cite{Gammie2008}. Exploiting forward body biasing (FBB), it is possible to increase the operating frequency of a device avoiding significant growth of dynamic power. 
%
%This process makes FBB suitable for compensation of variations causing degradation of the operating frequency. On the other hand, reverse body biasing (RBB) allows to significantly reduce leakage power where the process or operating conditions allow the devices to run faster than the target frequency, but with excessive leakage power \cite{Rossi2015a}.
%
%Similarly, temperature compensation can be achieved through voltage scaling and body biasing \cite{Kumar2008a}. 


%The majority of the works focusing on temperature effects target high performance devices that are subject to self-heating \cite{Oh2012a}. These devices necessitate the mitigation of the effects of temperature variation to avoid excessive leakage power dissipation that may lead to thermal runway. However, these works demonstrated the ability to compensate only for relatively small temperature ranges, not representative of the huge amount of scenarios enabled by ULP applications. Indeed, although self-heating does not affect ULP devices due to their extremely small power consumption, compensation of ambient temperature is crucial in this domain as well \cite{Alioto2012a}. 


%In this work, we analyze %for the first time 
%the capabilities of UTBB FD-SOI (Ultra Thin Body and Box Fully Depleted Silicon On Insulator) technology in compensating process variations in the ULP domain by means of on-chip Process Monitor Boxes (PMB) coupled with on-chip Body-Bias Generators (BBG). 
%To demonstrate this potential on real silicon we utilize a test vehicle consisting of an ULP cluster of processors operating in near threshold fabricated in 28nm UTBB FD-SOI technology. The compensation technique exploits one of the unique features of the UTBB FD-SOI technology: the ability to use the wide-range body bias to change the transistors voltage threshold. Body-Bias Generators allows to modulate the $V_{bb}$ in a wide range, theoretically from \SI{-3}{\volt} to $V_{dd}/2$ + \SI{300}{\milli \volt}.

The aim of this work is to \textit{i)} explore the wide-range body biasing capabilities of UTBB FD-SOI (Ultra Thin Body and Box Fully Depleted Silicon On Insulator) technology \textit{ii)} exploit on-chip Process Monitor Boxes (PMB) coupled with on-chip Body Bias Generators (BBG) to implement a performance-aware body biasing strategy that maximize the energy efficiency of the system. We demonstrate the proposed solution on silicon, a test vehicle composed of an ULP cluster of processors operating in near threshold, fabricated in 28nm UTBB FD-SOI technology. In this work we exploit the full body bias range: body-Bias generators allow to practically modulate the $V_{bb}$ from \SI{-1}{\volt} to $V_{dd}/2$ + \SI{300}{\milli \volt}. The proposed approach can be implemented both in hardware and software, enabling more advanced power management strategies.

%The main contribution introduced by this work is a general methodology, suitable to be implemented both in software and hardware, which enables advanced power management strategies. We start our work by studying the correlation between the output of the PMB and the actual maximum performance of the chip on the whole body-bias range; technical limitations practically reduce the body-bias range (from \SI{-1}{\volt} to $V_{dd}/2$ + \SI{300}{\milli \volt}). As successive step, we derive a general device-dependent linear model to predict the maximum frequency at each operating point. Our exploration covers the following set of OPs: $V_{dd}$ = \{\SI{0.5}{\volt},\SI{0.7}{\volt},\SI{0.9}{\volt}\} and for each supply voltage T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}. 

%Once the model's parameters have been obtained, we estimate the maximum error, finding that it is never higher than the 7\%. Then, we propose a methodology exploiting additional body-bias voltage margins to reduce it. Finally, we provide an evaluation of the overhead that this methodology causes on the global power consumption; we quantify it as the ratio between the additional leakage caused by the FBB margin and the global power consumption. The main result of this work is to show that temperature-induced variation compensation can be done by increasing the power consumption budget by less than 10\%. We derive, as last step, a more general methodology to compensate also process variations, with a worst-case overhead lower than 17\% in practical use case.

As a preliminary step, we calibrated the Process Monitoring Blocks by studying the correlation between their frequency measurement and the actual maximum frequency of the chip against the whole body-bias range.
This first step allows to properly model the response of the sensors, in particular we observed that the calibration model is a simple linear function. Our exploration covers the following set of OPs: $V_{dd}$ = \{\SI{0.5}{\volt},\SI{0.7}{\volt},\SI{0.9}{\volt}\} and for each supply voltage T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.
We quantified the error associated to the on chip measurement from PMBs in different conditions, finding that is always lower than 7\%.

We then propose a methodology exploiting additional body bias voltage margins to cancel the sensor's performance over estimations, for a single chip, at T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}. We measure the overhead on the leakage current caused by such body bias margins demonstrating that is lower than 10\%. We generalize the methodology deriving a multi-chip model, as in the previous case we quantify the mismatch between the model's maximum frequency prediction and the actual maximum frequency of the devices.

We implemented a software controller module employing the derived models to automatically probe maximum chip performance and properly tuning the body bias voltage to achieve a target frequency. We demonstrate the controller's operation by changing the temperature of the chip and observing the related body bias voltage adjustment. 

        %With respect to traditional bulk technology, UTBB FD-SOI technology enables an extended range of body bias and a better electrostatic control, that provides 85mV/V of threshold voltage/body bias voltage modulation. Starting from measurements on a multi-core system fabricated in 28nm UTBB FD-SOI technology we fit a compact model to extensively evaluate supply voltage and body biasing as knobs for compensation of temperature variations in the ULP domain.
        
        %Classical models suitable for describing the impact of physical parameters (i.e. Temperature. Voltage Supply and Body-Bias) on the performance and energy-efficiency of CMOS digital circuits shows severe limits when applied to ULP devices\cite{MARKOVIC_IEEE_2009}. Indeed classical models uses different model templates for describing super-threshold and near-threshold operating regions with discontinuities in the interface in between the two regions. Ambient temperature as well as body-bias at the macro-scale can be seen as changes to the overdrive voltage: moving the device from one operating region to the other. As a result empirical fitting of compact models which learns these dependencies are subjected to numerical errors. Recently new trans-regional models have been proposes based on EKV and polylogarithm models\cite{MARKOVIC_IEEE_2009}\cite{Poly}. In this paper we take advantage of these templates for fitting a compact model of the power and performance of a real silicon testchip under a large set of body-bias, voltage supply and ambient temperatures. We then used this model to compensate the Ambient Temperature variation.
        
        %Previous works on FD-SOI technology leverage the high performance flavour of the technology (flip well) that exploits full range (0V - 3V) forward body bias (FBB) to dramatically boost performance \cite{JACQUET_JSSC_2014} \cite{FRISBEE_ISSCC_2012}. In this work, we focus for the first time on the low-leakage flavour of the technology (conventional well) where a theoretical reverse body-biasing (RBB) up to -3V and a forward body-biasing (FBB) up to [VDD/2 + 300 mV] can be applied. Supporting both RBB and FBB, conventional well technology brings a lot of flexibility in terms of process and temperature compensation and it is very well suited for ULP applications due to its low leakage power consumption. 

%Remainder of this paper is organized as follows. Section \ref{overview} describes the chip used as test vehicle and the Process Monitor Boxes. Section \ref{sec:setup} describes the experimental setup, as well as the measurements performed to characterize the devices and extract the empirical models for the Frequency and Leakage current. Section \ref{analysis} provides a description of the analysis performed on the PMB sensors. Section \ref{temperature} describes the methodology used to compensate temperature variations.
%Section \ref{process} provides a description of the same methodology applied to the process variations compensation.
%Section \ref{sec:overhead} introduces a discussion of the results achieved by this methods, as well as a discussion of the overhead introduced by the two different compensations. Finally, section 6 gives some concluding remarks.

Remainder of this work is organized as follows. Section \ref{overview} describes the chip used as test vehicle and the Process Monitor Boxes.
Section \ref{sec:setup} describes the experimental setup and the measurements performed to characterize the devices and extract the empirical models for the Frequency. Section \ref{analysis} provides a description of the analysis performed on the PMB sensors. Section \ref{temperature} describes the proposed methodology used to compensate temperature variations. Section \ref{process} provides a generalization of the methodology to compensate also process variations. Section \ref{sec:controller} provides details on the implementation of the body-bias controller. Section \ref{sec:overhead} introduces a discussion of the results achieved, as well as a discussion of the overhead. Finally, section \ref{sec:conclusion} gives some concluding remarks.


==> Content/N02_overview.tex <==
\section{PULPv3 SoC}
\label{overview}

Parallel Ultra-Low-Power platform \cite{
Conti2015} version 3 (PULPv3) \cite{Rossi2017} is a multi-core SoC for ULP applications operating in near-threshold to achieve extreme energy efficiency on a wide range of operating points. The SoC is built around a cluster featuring four cores and \SI{64}{\kilo byte} of L2 memory. The cores are based on a highly power optimized micro-architecture implementing the OpenRISC-32bit ISA featuring 1kB of private instruction cache each. The cores do not have private data caches, avoiding memory coherency overhead and increasing area efficiency, while they share a L1 multi-banked Tightly Coupled Data Memory (TCDM) acting as a shared data scratchpad memory. The TCDM features 8 2kB SRAM  banks connected to the processors through a single clock latency non-blocking interconnect, implementing a word-level interleaved scheme to minimize banking conflict probability. Off-cluster (L2) memory latency is managed by a tightly coupled DMA featuring private per-core programming channels, ultra-low programming latency and lightweight architecture optimized for low-power and high transfer efficiency. In \figurename{\ref{fig:archi}} is shown the architecture of the system while \figurename{ \ref{fig:micro}} shows a micrograph of the chip. 

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/micrograph}
    %\missingfigure[figheight=7cm]{architecture of the SoC}
    \caption{This figure shows a micrograph of the chip and the main features.}
    \label{fig:micro}
\end{figure}

Advanced power management is enabled by three different power domains: \textit{i)} The "Safe Voltage Domain") hosting the Frequency Locked Loop generators, the two Body-Bias Generators for the SoC and Cluster regions, the PMB Controller and additional infrastructural control logic \textit{ii)} The  "SoC Body-Bias Domain" \textit{iii)} The "Cluster Body-Bias Domain". Each domain is monitored by a PMB, which will be described in the next section. In our tests, we will focus only on the Cluster Domain, applying $V_{bb}$ = \SI{0}{\volt} to the other body-bias domains.

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/PULPv3.png}
    %\missingfigure[figheight=7cm]{architecture of the SoC}
    \caption{Architecture of PULPv3 system.}
    \label{fig:archi}
\end{figure}



\subsection{Process Monitor Boxes}

A Process Monitor Box (PMB) is as an on-chip sensor based on ring oscillators, connected to the system through a digital interface, which provides a measurement of the maximum frequency achievable by the device. These sensors are designed and optimized to behave consistently with the other library logic gates, attempting to emulate all the parasitic effects induced by temperature's and process' variations. More specifically, in our design we used PB0 sensors designed to monitor RVT P0 cells. \figurename{ \ref{fig:PMB}} sows in detail the PMB sensor architecture and the digital interface to read the measurement.

\subsection{Body-Bias generators}

The body bias voltage is modulated thanks to a fully integrated body-bias. Such body bias generator is capable to apply a fine-grain body-bias voltage with a minimum step of \SI{50}{\milli \volt} and can cover a voltage range from \SI{-1.5}{\volt} to $V_{DD}/2$ + \SI{300}{\milli \volt}. This device has been designed to target ULP system on chips\cite{Blagojevic2016} and further optimized to maximize the energy efficiency\cite{Rossi2017}. The generator is programmed through a series of memory mapped registers and can independently bias with different voltages the Nwell and the Pwell of the transistor.


\section{Experimental Setup}
\label{sec:setup}

To compare the ambient temperature and process variations on next generation ULP devices, we conducted a large data acquisition test directly on the PULPv3 prototypes, measuring power and performance metrics at the different corner cases. Based on the measurement results, we have derived a set of empirical models to describe the dependency of the performance metrics to the physical parameters, compensation knobs and environmental conditions. This models will be discussed in the next sections of the paper.

The measurements described are performed with an Advantest SoCV93000 tester system, in connection with a Thermonics 2500E temperature forcing system, able to force an environment temperature ranging from \SI{-80}{\celsius} to \SI{220}{\celsius}. 
Since we are interested in using the body-biasing voltage as independent variable both for temperature and process variations compensation, we structured the measurements as follows: \textit{i)} We defined the operating point (OP) in terms of \{Supply voltage $V_{dd}$ , Temperature\}, where $V_{dd}$ = \{\SI{0.5}{\volt},\SI{0.7}{\volt},\SI{0.9}{\volt}\} and T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}; \textit{ii)} For each OP we swept the body-biasing voltage ($V_{bb}$) in the range \SI{-1}{\volt} to $V_{dd}/2$ + \SI{300}{\milli \volt} using the Body-Bias Generator, and we measured: the leakage power ($P_{LKG}$), the active dynamic power ($P_{DYN}$), the total power ($P_{TOT}$) and maximum frequency ($F_{MAX}$) achievable by the device.
More specifically, we measured the active dynamic power ($P_{DYN}$) as the difference between the Total Power ($P_{TOT}$) and the leakage power ($P_{LKG}$). The Total Power ($P_{TOT}$) has been measured as the power consumption when the device is executing an arithmetic loop (Matrix Multiplication), and the Leakage Power ($P_{LKG}$) as the power consumption when the device is not clocked. We extracted the maximum operating frequency ($F_{MAX}$) by means of a carefully crafted benchmark, able to trigger the most critical paths\footnote{The critical path, identified by the timing analysis in the communication between the cores and the scm memory, was massively triggered by the algorithm we used as benchmark to measure the maximum frequency.} of the circuit. We verified that the result of the arithmetic operation was returned with the correct timing, and the End-Of-Computation\footnote{Physical output pin of the device which certifies that the system completed all the operations and properly entered a known final state.} signal was properly asserted. As cross-check, we verified that the arithmetic loop returned a valid check-sum.





==> Content/N03_temp_comp.tex <==
\section{PMB characterization}
\label{analysis}

%The first part of the methodology proposed in this paper has the aim to exploit the run-time maximum frequency measurement, performed with the test equipment, to determine the actual maximum frequency of the chip. In parallel, by observing the PMBs' output, it is possible to find a correlation between the actual maximum frequency and the one predicted by the PMBs.
%Once the equation to translate the PMB frequency estimation in $F_{Max}$ has been found, given a target frequency specified by the application and depending on the $V_{dd}$, the body-bias voltage can be finely regulated to fill the performance's gap.

First part of the analysis focuses on the characterization of the performance monitoring blocks placed in the power domain of interest, that is the one hosting the core's cluster. The aim of this step is to obtain a model allowing to correctly interpret the response of the frequency probes (PMBs). To obtain the model, we simultaneously observed both the response of the PMBs ($F_{pmb}$) and the maximum chip's frequency measured on the testing equipment ($F_{max}$). This characterization has been done against the entire body bias range.\tablename{ \ref{tab:meas_details}} shows more details regarding the measurement's operating conditions.

\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c}
        PULP $V_{DD}$ & $V_{BB}$ & $T_{op}$ & Process corner\\
        \SI{0.7}{\volt} & \SI{-1}{\volt} to \SI{650}{\milli \volt} & \SI{25}{\celsius} & Typical 
    \end{tabular}
    
    \caption{Measurement's operating conditions}
    \label{tab:meas_details}
\end{table}

Since the focus of this step is to obtain a preliminary evaluation of the PMB's accuracy, the temperature is externally enforced by the testing equipment and assumed as known. The measurements in this phase are referred to a single chip, this allows   to exclude the process variation as possible source of error because we know if the device in exam is a \textit{Fast}, \textit{Typical} or \textit{Slow} one. \figurename{ \ref{fig:frequency}} reports the measurement of the $F_{pmb}$ and $F_{max}$ versus $V_{BB}$ for a typical device supplied at \SI{0.7}{\volt}.
%For the sake of simplicity, in this section we will not consider the variations introduced by the process; accordingly with this assumption, we assume to use a model calibrated on the specific chip. In other words, the correlation between the value provided by the PMB sensor and the maximum achievable frequency of the chip is calculated for the specific device under test. \figurename{\ref{fig:frequency}} shows on the same plot the maximum frequency measured with the test equipment and the PMB estimation for a typical device at \SI{0.9}{\volt} and \SI{25}{\celsius}

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{C550925frequency}
    %\missingfigure[figheight=7cm]{correlation's linearity for different chips}
    \caption{This plot compares the maximum achievable frequency and the PMB frequency estimation for a typical chip at \SI{0.9}{\volt} and \SI{25}{\celsius}.}
    \label{fig:frequency}
\end{figure}

%As shown in \figurename{\ref{fig:correlation}}, the relationship between the values provided by the PMB and the maximum frequency of the device can be modeled with a simple affine function\footnote{ The $C_{corr}$ parameter represents the ratio between the delay of the critical paths and the minimum delay determining the frequency of the oscillator inside the PMB. The $F_{0}$ parameter is an offset related to the critical path of the circuit.} (Equation \ref{eq:model}).

In the second phase of the PMB's characterization we evaluated the correlation between $F_{pmb}$ and $F_{max}$. As shown in figure \figurename{ \ref{fig:correlation}}, the model we found is the linear function reported in \ref{eq:model}. In \figurename{ \ref{fig:correlation}} is reported the linear fit's plot of the data.

\begin{equation}
\label{eq:model}
    F_{max} = C_{corr} F_{pmb} + F_{0}
\end{equation}

%\tablename{ \ref{tab:model}} shows the parameters of the linear fit at the three OPs for a single device. Notice that the $C_{corr}$ is always lower than 1, which means that the maximum frequency of the circuit is always lower than the the one generated inside the PMBs. The R-Square parameter is always equal or higher than 0.995, indicating that the model properly describes the data's trend.

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{C550925correlation2}
    \caption{This plot shows the relation between the maximum frequency and the PMB frequency estimation for a typical chip at \SI{0.9}{\volt} and \SI{25}{\celsius}. The data have been fitted with a linear model, the parameters of the fit are: y=mx+q where m=0.6 and q=8.7, R-Square (COD) = 0.995.}
    \label{fig:correlation}
\end{figure}

We repeted the same measurements in different operating conditions proving the robustness of the model: \tablename{ \ref{tab:model}} reports the parameters of the model.

\begin{table}[hbt]
    \centering
    \begin{tabular}{r|c|c|c}
        $V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\
        $C_{corr}$ & 0.6 & 0.59 & 0.47 \\
        $F_{0}$ & 8.72 & 5.19 & 3.21\\
        R-Square & 0.995& 0.998 & 0.998\\
    \end{tabular}
    \caption{Parameters of the model for a typical chip at three different supply voltages and \SI{25}{\celsius}.}
    \label{tab:model}
\end{table}

%The equation we use to correlate the maximum frequency with the PMB frequency estimation, as well as other techniques used in other work, can be affected by errors.
%In our case the error is represented by the residuals of the measurements with respect to the fitting curve. The maximum residual we report for the correlation model, at fixed Operating Point, and for a single device, is the 3\%. Comparable errors are reported also in \cite{Beigne2015}, a similar study performed on a DSP architecture implemented with the same FD-SOI technology and exploiting a performance monitor system based on Timing Fault Sensors (TMFLT).
As a final step for this preliminary PMB characterization we estimated the model's error, which is represented by the residuals of the measurements with respect to the fitting curve. The maximum residual we report for the correlation model for a single device is the 3\%. Comparable errors are reported also in \cite{Beigne2015}, a similar study performed on a DSP architecture implemented with the same FD-SOI technology and exploiting a performance monitor system based on Timing Fault Sensors (TMFLT).


%The presence of the model's error, that is a frequency uncertainty affecting the Maximum frequency estimation, can be compensated by means of additional forward body-bias. Notice that the $V_{bb}$ margin added to compensate the model's uncertainty, is conceptually different from the $V_{bb}$ regulation to achieve a target frequency. The approach used to compensate the error will be discussed in the next section.


\section{Temperature Variations}
\label{temperature}

%The model we propose for the temperature-induced variation compensation is a generalization of the approach we described for a single operating point. To derive a more general fitting function, we performed the same data analysis on the entire data set (multiple OPs) introducing hence an additional degree of freedom. Thanks to this analysis, we obtained a general equation describing all the operating points for a single device. 
%In \figurename{\ref{fig:perchip_model}} is reported the entire set of measurements performed at different voltages and temperatures for a typical device. The red solid line, which is described by the equation \ref{eq:model}, represents the general model fitting the data. Table \ref{tab:model_temp} reports the parameters of the model in this case as well as the R-Square.

Once the robustness of the PMB model has been proved in a given operating condition, it is possible to generalize the analysis to cover multiple operating points. The measurements described in this section are performed on a single chip, supplied with a given voltage ($V_{DD}$), at multiple temperatures. The approach is the same we followed in the previous case, the only difference is that the fitted data are now related to three different temperatures, specifically T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.

\figurename{ \ref{fig:perchip_model}} shows the global linear fit, The red solid line, which is described by the equation \ref{eq:model}, represents the general model fitting the data. Table \ref{tab:model_temp} reports the parameters of the model in this case as well as the R-Square. As in the previous case, we evaluated the error,\figurename{ \ref{fig:perchip_error}} shows the residuals with respect to the fitting curve. As expected, a model which fits data belonging to measurements at various temperatures is affected by a larger error. this phenomenon is caused by the fact that we are assuming that the maximum frequency is limited only by the PMB related to the PMOS transistors, which is usually slower than PMB related to the NMOS ones. Correlation between the maximum frequency of the device and a linear combination of both PMB could improve the accuracy. 

\begin{table}[htb]
\centering
    \begin{tabular}{r|c}
        $V_{dd}$ & \SI{0.7}{\volt}\\
        $C_{corr}$ & 0.59 \\
        $F_{0}$ & 5.42 \\
        R-Square & 0.996\\
    \end{tabular}
    \caption{Parameters of the model fitting the data for a single chip, at a given supply voltage, at three different temperatures.}
    \label{tab:model_temp}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width = \columnwidth]{temp_with_bands}
    \caption{In this plot are shown all the measurements performed at a single supply voltage $V_{dd}$ = \SI{0.7}{\volt} and three different temperatures T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}. The red solid line represents the general model to correlate the output of the PMB sensor with the maximum frequency of the device, which is the global fitting curve for the entire data-set.}
    \label{fig:perchip_model}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width = \columnwidth]{error-temp-new}
    \caption{This plot shows the distribution of the relative error versus the maximum frequency when the general model is used to convert the PMB output value in $F_{max}$.}
    \label{fig:perchip_error}
\end{figure}





==> Content/N04-5_body-bias.tex <==
\section{Body-Bias Model}
The final goal of this study is to develop a performance-aware body bias regulation system, to this end, it is necessary to derive a model which links a variation of the $V_{BB}$ to the $F_{max}$ variation. Once the relationship between this two parameters has been obtained, given a performance gap to be compensate, it is possible to determine the necessary amount of body bias voltage to do it.

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{freq_to_vbb07}
    \caption{This plot shows the relation between the maximum frequency of a typical device and the body-bias voltage at three operating points: Vdd = \SI{0.7}{\volt} and T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.}
    \label{fig:freqvbb}
\end{figure}

It is very important to note that the use of body-bias for this application is twofold: \textit{i)} in an ideal case, that is assuming no errors on the $F_{max}$ estimation, $V_{BB}$ represents the knob to simply change the performance of the device \textit{ii)} in a context where $F_{max}$ is affected by uncertainty because of the reasons previously described, $V_{BB}$ margins can be used to compensate $F_{max}$ over-estimations; in other words, all those conditions where the $F_{max}$ measurements residuals are negative. \figurename{\ref{fig:freqvbb}} shows the relationship between $F_{max}$ and $V_{BB}$ at different temperatures.
%Starting from the error estimation, since we assume to know the supply voltage at every OP, we used the empirical model that links the frequency and the body-bias voltage to convert the frequency error in a forward body-bias margin to add to the $V_{bb}$ regulation. Notice that we are interested in aligning the maximum frequency achievable by the chip to the target one, therefore we need to compensate only for negative frequency errors. 
%In other words, we will compensate those conditions where the general model overestimates the real performance of the device.

Despite the curve shifts with temperature, if we consider the relative frequency variation, we can simplify the body bias model approximating the curve with a linear function having $5\%/\SI{100}{\milli \volt}$ as slope (\figurename{ \ref{fig:freqvar}}).
Table \ref{tab:perf_gain} shows the same analysis at different voltage operating points.

\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c}
        PULP \SI{0.5}{\volt} & \SI{0.7}{\volt} & \SI{0.9}{\volt}\\
        $11\%/\SI{100}{\milli \volt}$ & $5\%/\SI{100}{\milli \volt}$& $3\%/\SI{100}{\milli \volt}$
    \end{tabular}
    
    \caption{Body bias induced performance gain}
    \label{tab:perf_gain}
\end{table}
%As shown in \figurename{\ref{fig:freqvbb}}, the relationship between the frequency and the body-bias voltage shifts with the temperature, however, as shown by the plot in \figurename{\ref{fig:freqvar}}, once the supply voltage has been fixed, the relative frequency variation (in the forward body-bias region) can be considered in first approximation as temperature-independent; because the three curves are superimposed.

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{frequency-variation}
    \caption{In this plot is represented the relative frequency variation versus the body-bias voltage, with respect to the $V_{bb}$ = \SI{0}{\volt} condition. The operating points are: Vdd = \SI{0.7}{\volt} and T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.}
    \label{fig:freqvar}
\end{figure}

This model allows to compute the additional body bias margin required to compensate the measurement's errors described in the previous sections. Assuming to compensate the model's uncertainty caused by temperature, which was the 3\% at \SI{0.7}{\volt}, we need to add a margin on $V_{BB}$ of \SI{75}{\milli \volt}.

It can be noted that body bias margins can be summed as independent contribution to compensate different errors of the models. Assuming to use a model which is process-unaware and temperature-unaware, hence affected by an error of 7\% + 3\% respectively, these errors can be compensated with the sum of the two independent body bias margins\cite{Kumar2008a}.
%Starting from this assumption, the amount of additional forward body bias that allows to neglect the effects of temperature variation can be calculated exploiting the relative frequency versus body-bias voltage relation reported in \figurename{\ref{fig:freqvar}}, which is the frequency-normalized inverse of \figurename{\ref{fig:freqvbb}}. To give an example, assuming that we want to compensate the error at \SI{0.9}{\volt} shown in \figurename{\ref{fig:perchip_error}}, that is the 3\% in the worst case, we need to consider a $V_{bb}$ margin of \SI{0.1}{\volt} (The amount of body-bias is derived by the curves in \figurename{\ref{fig:freqvar}}). Notice that the additional amount of $V_{bb}$ causes an increase in the leakage current, hence additional leakage power consumption; the overhead caused by this methodology will be discussed in section \ref{sec:overhead}.




%As anticipated in the previous section, we considered the variations introduced by the process and the variations introduced by the temperature as separated. As demonstrated in \cite{Kumar2008a}, the additional body-bias voltage used to reach the target frequency, plus the margin to compensate the uncertainty of the model, can be summed to the fraction of $V_{bb}$ used to compensate process' variations as independent contributions.

==> Content/N04_process_comp.tex <==
\section{Process variations}
\label{process}

%In this section we generalize the methodology we proposed to reduce the sensitivity to temperature' variations to compensate also process' variations.
Operating temperature is not the only factor affecting device's performance operating in near threshold. In this section we will present a short discussion on the performance variance among different chips fabricate in the UTBB FD-SOI technological node caused by different process corners. Then, we will show how the performance monitoring methodology described so far can be further generalized to cover also multiple chips belonging to various process corners. Particular attention should be given to the nature of the performance variation related to the technological process, the variations introduced by the process can be classified in two types: \textit{i)} The Inter-chip variations, that can be observed in terms of performance gaps between different devices, as shown in \figurename{ \ref{fig:frequency_distribution}} \textit{ii)} Intra-chip variations, as demonstrated by \cite{Zandrahimi2016}, resulting in different first N critical path, that can affect the consistency between the behaviour of the circuit and an on-chip performance monitor, confirmed also by our analysis.

%Here, we discuss the results of the analysis performed on a population of 8 different chips. In figure \figurename{\ref{fig:process_model}} are reported the correlation data of all the chips in exam, for a given OP. Notice that the variations introduced by the process can be classified in two types: \textit{i)} The Inter-chip variations, that can be observed in terms of performance gaps between different devices, as shown in \figurename{\ref{fig:frequency_distribution}} \textit{ii)} Intra-chip variations, as demonstrated by \cite{Zandrahimi2016}, resulting in different first N critical path, that can affect the consistency between the behaviour of the circuit and an on-chip performance monitor, confirmed also by our analysis.

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{frequency_distribution}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{Normalized distribution of the maximum frequency for the entire population of 48 chips at \SI{0.9}{\volt}, \SI{25}{\celsius}.}
    \label{fig:frequency_distribution}
\end{figure}

As in the case of one chip at multiple temperatures, the model has been obtained by performing a global fit on the data related to chips belonging to different process corners, finding the best function describing them with minimum error; \figurename{ \ref{fig:process_model}} shows the PMB analysis related the chips in exams and the fitting curve.

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{multiple}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{In this plot are represented the data of 8 different chosen devices, the red solid line represents the fitting curve we assume as process-independent model.}
    \label{fig:process_model}
\end{figure}

Notice that also in this case the model is represented by the same linear function \ref{eq:model} shown previously. However, in this case the fitted data have a larger variability, as a consequence, we observed a larger error and lower R-square. Table \ref{tab:model_temp_process} shows the values of the parameters and the R-Square.
When the chip was fabricated the technology node was at a very early stage, according to what described in [XXX], the variance introduced by the manufacturing process is expected to decrease with the maturity of the process.

%As for the temperature variation compensation, we derived a general correlation model between all the chips. \figurename{\ref{fig:process_error}} shows the error when this model is used to convert the output of the performance monitor sensor. Also in this case the model is the one described by equation \ref{eq:model}, table \ref{tab:model_temp_process} reports the values of the parameters and the R-Square; notice that in this case the fitted data have a larger variability, resulting in a larger Prediction band and lower R-square.

\begin{table}[htb]
\centering
    \begin{tabular}{r|c}
        $V_{dd}$ & \SI{0.7}{\volt}\\
        $C_{corr}$ & 0.614 \\
        $F_{0}$ & 6.86 \\
        R-Square & 0.88\\
    \end{tabular}
    \caption{Parameters of the model fitting the data related to chips belonging to different process corners, at a given supply voltage, at three different temperatures.}
    \label{tab:model_temp_process}
\end{table}

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/multi_error_vdd2.png}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{This plot shows the distribution of the relative error versus the maximum frequency when the process-independent model is used to convert the PMB output value.}
    \label{fig:process_error}
\end{figure}

%To generalize the model and compensate the error, as in the previous section, we derived the function that links the $v_{bb}$ with the relative frequency change at different supply voltages. As shown in figure \figurename{\ref{fig:relative-freq}}, the sensitivity of the frequency with respect to the body-bias, in the forward body bias region, decreases when the supply voltage increases. Starting from this assumption, we can assess that, using a $V_{bb}$ margin to compensate a frequency gap at \SI{0.9}{\volt}, at minimum the same frequency gap will be compensated also for lower supply voltages. More specifically, we can state that the frequency sensitivity to body-bias voltage is always higher than 10\%/\SI{100}{\milli \volt}. Using this more general model, as expected, we obtained higher frequency errors (\figurename{\ref{fig:process_error}}).

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width = \columnwidth]{relative-freq-allV}
%    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max %freq on 10 chips}
%    \caption{The graph shows the Relative frequency sensitivity to the $V_{bb}$ at %different operating points.}
%    \label{fig:relative-freq}
%\end{figure}






==> Content/N05_overhead.tex <==
\section{Methodology's Overhead}
\label{sec:overhead}

%The methodology we propose uses the forward body-biasing to compensate the uncertainties in process monitor readings. Since the $V_{bb}$ has a straightforward effect on the leakage current, hence on the leakage power consumption, it is important to quantify the overhead introduced by the body-bias margins. As it is well known, the higher is the frequency of the system, the more dominant is the dynamic power consumption with respect to the leakage power. Hence, the overhead decreases as the target frequency increases, since only the leakage power changes when the FBB is applied.
%Notice that we define the overhead as the additional leakage power with respect to the global power consumption, assuming to calculate it in the most common operating condition for a near-threshold processor, that is when the system is running at the maximum achievable frequency, given a supply voltage.

The compensation methodology we propose is based on the application of forward body bias to compensate model's frequency error. As it is well known, FBB has a direct influence on the leakage current of a circuit, hence it is important to quantify the overhead associated with the additional body bias margins. Specifically, we defined the overhead as the ratio between the additional leakage caused by the body bias margin and the leakage current of the circuit. How the additional leakage current affects the global power consumption strongly depends on the dynamic power consumption (i.e operating frequency) of the circuit, hence the overhead will be provided with respect to the leakage current.

%The following tables report the worst case overheads at three different conditions: \textit{i)} when the Process-unaware model is used \textit{ii)} when it is possible to calibrate the model on the single chip \textit{iii)} when we can fully characterize the operating point knowing also the temperature.

The overhead presented in this section refers to the three different models derived in the previous sections. More specifically, to the cases where the supply voltage is known and \textit{i)} the process corner and the temperature are known \textit{ii)} the process corner is known and the temperature is unknown \textit{iii)} both temperature and process corner are unknown.

%Assuming to probe also the temperature, the only error affecting the model is the one given by the fitting curve, which is the 5\% in the worst case (\SI{0.5}{\volt}), resulting in a worst case overhead of the 3\%.

In the first case, the worst case model's error to compensate with additional body bias margin is the 5\% ($V_{DD} = \SI{0.5}{\volt}$), that is the biggest residual between the measurements and the curve fitting the data of a single chip at a single temperature. We measured that the additional leakage caused by the body bias margin added to correct such error represents the 3\% of the global power consumption.

If we consider the leakage current associated with margins needed to correct the errors of the temperature independent model, we can observe that the overhead is the one reported in Table \ref{tab:temp}.
%When the model can be calibrated on the specific device, it is possible to reduce the error in the maximum frequency estimation approximately of a factor of 3. Table \ref{tab:temp} shows the results in terms of frequency errors and overhead in this condition.
\begin{table}[hbt]
    \centering
    \begin{tabular}{r|c|c|c}
        $V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\
        $F_{err}$ & 3\% & 4\% & 7\% \\
        $Leakage overhead$ & 19\% & 24\% & 39\%\\
    \end{tabular}
    \caption{Frequency error and power consumption overhead for temperature effect compensation.}
    \label{tab:temp}
\end{table}

%When only the supply voltage is known, it is necessary to compensate temperature and process variations, as a consequence, the frequency error in the estimation of the maximum one is high and also the power consumption overhead. Table \ref{tab:temp-proc} summarize the results at three different operating voltages.
Table \ref{tab:temp-proc} reports the overhead when the third model, that is the process corner unaware temperature-unaware model. As expected, the higher is the uncertainty of the model, the wider is the body bias safety margin required to use the model, and also the higher is the associated overhead because of the higher leakage current.

\begin{table}[hbt]
    \centering
    \begin{tabular}{r|c|c|c}
        $V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\
        $F_{err}$ & 6.6\% & 9.7\% & 25\% \\
        $Leakage overhead$ & 41\% & 65\% & 260\%\\
    \end{tabular}
    \caption{Frequency error and power consumption overhead for temperature and process variation compensation.}
    \label{tab:temp-proc}
\end{table}



            %\figurename{\ref{fig:overhead}} shows the trend of the overhead for different supply voltages, when the temperature is equal to \SI{80}{\celsius}, hence when the influence of the leakage on the dynamic power is maximum.
            
            % \begin{figure}[htb]
            %     \centering
            %     \includegraphics[width = \columnwidth]{overhead_temp}
            %     %\missingfigure[figheight=7cm]{overhead}
            %     \caption{Worst case overhead caused by the temperature effect compensation at three different operating points: $V_{dd}$ = \{\SI{0.9}{\volt} , \SI{0.7}{\volt} , \SI{0.5}{\volt}\}.}
            %     \label{fig:overhead}
            % \end{figure}
            
            % Concerning the overhead to compensate process variations, it can be calculated as an additional contribution to the temperature compensation's overhead. \figurename{\ref{fig:overhead_gen}} shows the global overhead versus the target frequency 
            
            % \begin{figure}[htb]
            %     \centering
            %     \includegraphics[width = \columnwidth]{global_overhead}
            %     %\missingfigure[figheight=7cm]{overhead}
            %     \caption{Worst case overhead including the compensation of both the temperature and process variations.}
            %     \label{fig:overhead_gen}
            % \end{figure}


==> Content/N06_frequency_tracking.tex <==
\section{Controller operation}

\subsection{Frequency Tracking}
In the following we present a controller working example. \figurename{ \ref{fig:control_op}} shows the $V_{BB}$ regulation operated by the controller when the frequency set-point is changed to different values.

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{controller_op}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{controller operation}
    \label{fig:control_op}
\end{figure}

The first set-point, 192MHz, is very close the maximum frequency of the device. In this condition the controller is applying a very small amount of body-bias, since the system is already capable to run at the requested frequency, without additional forward body-bias. The only body bias voltage applied ($V_{BB} \neq 0$) is the body bias margin. When 230MHz are requested as set-point, the controller applies a forward body-bias voltage of approximately 450mV; applying a strong forward body bias, the system is now capable to run at 230MHz. On the contrary, when a slow frequency is set as set-point, 96MHz, the controller applies aggressive reverse body-bias to reduce leakage power as much as possible. Finally, when the setpoint is restored to 192MHz, the system stops applying revers body bias and apply nominally zero body bias plus safety margin.

\subsection{Temperature tracking}

In this section we show another working example. In this case the controller is used to guarantee a 170MHz frequency target against environmental temperature changes. We present in the following the behaviour of temperature (\figurename{ \ref{fig:temp_time}}), leakage (\figurename{ \ref{fig:leak_time}}) and body-bias voltage (\figurename{ \ref{fig:vbb_time}}).

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/bodybias_time.png}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{This picture shows the body-bias voltage modulation operated by the controller during temperature changes}
    \label{fig:vbb_time}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/temp_time.png}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{This picture shows the environmental temperature variation}
    \label{fig:temp_time}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/leak_time.png}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{This picture shows the leakage current which is kept under control by the body bias controller}
    \label{fig:leak_time}
\end{figure}

From the leakage current's plot it is clear that the controller is compensating the environmental temperature increase applying a reverse body-bias voltage. On the contrary, when the temperature decreases, to guarantee the requested target frequency the controller applies a forward body-bias voltage to boost the maximum performance of the chip.

==> Content/N07_controller.tex <==
\section{Body-Bias Cotroller}
\label{sec:controller}
%----------------------------------
%
% body bias controller
%
%---------------------------------
% 1. purpose of the controller
% 2. Feedback and actuator
% 3. models involved
% 4. empirical tuning
% 5. working example
In this section we will show how the models derived so far can be used in practical applications. More specifically, an accurate on-chip performance feedback, as well as the modeled behavior of the body-bias generator enable the building of software control systems; the structure we propose is a mixed Hardware-Software solution which properly set the cores' cluster Body-Bias voltage depending on the clock frequency set-point provided as input.

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/Controller_new.png}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{Body-bias controller}
    \label{fig:control}
\end{figure}

\subsection{Controller Modules}
The proposed Body-bias controller is composed of: \textit{i)} a feedback, \textit{ii)} a subtractor which computes the mismatch between feedback and set-point, \textit{iii)} a Proportional-Integrative-Derivative (PID) controller, \textit{iv)} an actuator fed with the PID controller's output; figure \ref{fig:control} shows a block diagram of the body bias control system.

The control system's \textit{feedback} module is divided in two main building blocks: \textit{i)} a hardware component, the previously mentioned PMB, which returns a raw maximum frequency estimation; \textit{ii)} the software model derived for the PMB, which allows to properly convert the raw output of the sensor in a clock frequency value. 

The \textit{PID controller} is a standard well-known control mechanism used in industrial control systems \cite{wikipediaPID}, the proposed Body-Bias control system  is entirely implemented in software and it is fed with the mismatch between feedback and set-point frequency.

The \textit{actuator}, as in the case of feedback module, is composed of two building blocks: the on-chip Body-Bias generator, paired with a software model which allows to determine the right amount of Body-Bias needed to fill the frequency gap between feedback and set-point.

\subsection{PID Tuning} 

The PID tuning is a process that can be done empirically.In the contex of this control task we decided to adopt a parameter set which minimizes the settling time while keeping under control undershoots. Notice that undershoots are critical for this kind of system, when the controller applies a too low body-bias voltage the probability of a system's failure dramatically increases, and the system is prone to irreversible errors.

As shown in Figure \ref{fig:control}, the entry point of the control system is the frequency set-point $F_{ref}$. The first operation performed by the controller is to measure the maximum frequency of the system. Once the output of the PMB module is ready, it is been converted in a frequency value, and it is compared with the input set-point obtaining the frequency mismatch. Then, the PID module is fed with the frequency mismatch and its output is sent to the body-bias software model. Finally, once the models computes the body-bias voltage to apply, it is used to set the body-bias generator to the new $V_{BB}$ value.




==> Content/N08_results.tex <==
\section{Results}

In this section we present results in terms of possible energy efficiency gain and leakage reduction when the body-bias controller is turned on. \figurename{ \ref{fig:leakage}} shows a comparison between the leakage current when \textit{i)} the controller is off and the leakage is not compensated against temperature \textit{ii)} the controller is on \textit{iii)} the ideal case where the leakage is compensated without additional body bias margins, hence assuming no error in the model converting the frequency estimation of the PMB. Notice that the influence of the leakage power on the global power consumption depends on the operating frequency of the device, in our measurements the controller is regulating the body bias to achieve a target frequency of 160MHz, which represents an optimal operating point, since the working frequency is close to the maximum one.

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/leakage_comparison_160MHz2}
    \caption{This plot whos the leakage current versus temperature, in the case when: \textit{i)} the controller is off and the leakage is not compensated against temperature \textit{ii)} the controller is on \textit{iii)} the ideal case where the leakage is compensated without additional body bias margins}
    \label{fig:leakage}
\end{figure}

\figurename{ \ref{fig:leakage}} also shows that the margin required to compensate process variations cause a big increase in the leakage current, in this context the effect on the global power consumption is not anymore negligible. However this problem can be solved by running a simple calibration procedure which determines if the chip is a \textit{Slow}, \textit{Typical} or a \textit{Fast} one. The benefit of the calibration procedure is to reduce the body bias margins to the ones related with temperature, cutting by a factor of 3 the overhead on the leakage current.

\figurename{ \ref{fig:power}} compares the power consumption of the entire chip, at different temperatures, both in the case when the body bias controller is turned on and off. As it is evident from the plot, the use of the body bias controller allows to increase the energy efficiency by a factor of 1.3X (at high temperatures)

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/power_new.png}
    \caption{Comparison between power consumption with and without the performance aware body bias controller}
    \label{fig:power}
\end{figure}





==> Content/N09_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work we demonstrated the body-biasing capabilities of the UTBB FD-SOI technology in compensating temperature and process variations.

We performed an analysis on the Process Monitoring Blocks to correlate the on-chip estimated maximum frequency to the actual performance of the device, hence we derived a calibration model for the sensors. We extended the model obtained at a single temperature to multiple temperatures to compensate the effect environmental temperature changes have on the performance of the device. Then we further extended the model to the case when the process corner is unknown, therating it as an uncertainty of the model. We found that the error in frequency estimation at single operating point is in the order of 3\% at \SI{0.7}{\volt}, 4\% in the case of multiple temperature and 9.7\% when the process corner is unknown. We developed a strategy to eliminate such frequency estimation error by over-compensating with selective body bias margins. in the final part of the analysis we quantified the overhead on the leakage current associated with the body bias margins, that is 24\% when the error is 3\%, 65\% when the model's error is 9.7\%, and 200\% when the process corner is unknown and the frequency estimation is affected by a 25\% of error.

Once the models have been obtained, we developed a closed loop control strategy for the body bias voltage based on a simple PID controller. We tested the models for the frequency estimation and the body bias in this context, demonstrating that an automatic body bias regulation can reduce with a minimum overhead leakage power consumption caused by temperature chenges by a factor of 2. Finally we evaluated the effect of the leakage reduction in a common operating context, demonstrating that our approach can introduce a 1.3X energy efficiency improvement on the global power consumption.
%We developed a methodology that provides run-time Maximum Frequency estimation by means of Process Monitor Boxes, enabling performance optimization policies exploiting body-bias regulation. We generalized the model to operate across all the allowed operating points in terms of supply voltage and temperature, for a single device, by means of a finely tuned body-bias-based temperature compensation. We proved that the error can be lower than the 3\% in the best case, and it can be kept below 7\% in the worst case. In this condition we measured an overhead in the global power consumption always lower than 5\%.
%We generalized the methodology to compensate also process variations proving that the overhead is lower than the 17\% in the worst case and lower than 10\% in the best case. We observed that having the possibility to probe also the temperature, the error can be reduced to 5\%, causing an overhead on the global power consumption lower than 3\%.


%In this work we demonstrated the extended reverse and forward body bias capabilities of UTBB FD-SOI technology in compensating for process and temperature variation in the ULP domain. We carried out the exploration on real silicon using as test vehicle an ULP full multi-core architecture operating in near threshold, fabricated for the first time using UTBB FD-SOI technology. From real measurements we derived a trans-regional compact model which relates ambient temperature, body bias and supply voltage to energy and maximum performance achievable by the device. This model is then suitable for finding the optimal body-bias and supply voltage which compensates for process and temperature variation. We demonstrated the unique capabilities of UTBB FD-SOI to compensate for temperature variation on the wide range of -40\textdegree C to 120\textdegree C exploiting body biasing, providing up to 15\% better energy efficiency with respect to compensation through adaptation of supply voltage only.

==> Content/N10-11_Embedded_setup.tex <==
\section{Embedded setup}



==> Content/Rebuttal_Letter.tex <==
\onecolumn
\section*{Response to the reviewers}
% General intro text goes here
We thank the reviewers for their critical assessment of our work. 
In the following we address their concerns point by point.

%{\parindent0cm 
%\textbf{Rebuttal letter}

%\textbf{Comments from the editors and reviewers:}

%\textbf{Reviewer 1:}

\reviewersection

\begin{point}
Hello,
I like the organization of this paper, and i fully agree with the conclusions of your work. However, I would find more details about the implementation body bias Generator (SECTION III).
\label{point:bb_details}
\end{point}

\begin{point}
Are the back bias generator dependent on the digital area capacitive load? What is the digital area range supplied by the BBG? Is your regulation sensible to  the Back Bias leakages  (VNW/VPW/SUB)?
\label{point:bb_details2}
\end{point}

\begin{reply}
\fix{}{To address \ref{point:bb_details} and \ref{point:bb_details2} we provided a more detailed description of the body bias generators. \fix{}{The BB gen has been designed to drive an area of \SI{1}{\milli\metre\squared}. For positive regulation of both wells the BB gen uses a push-pull approach. Negative regulation on the p-well is obtained by means of a dual phase charge pump. Two control loops allow to monitor the impact of the leakage and compensate for wells discharge. The comparators of the feedback use Resistive Digital to Analog Converters (DAC) as references. To reduce the power consumption of the BB gen to \SI{4.5}{\micro \watt}, its operation is duty-cycled, entering a sleep mode where only the leakage is monitored.
This paragraph has been integrated in section III, subsection 2.}}
\end{reply}

\begin{point}
In the text , it seems that the body bias generator can supply a VBB (VNW-VPW) step of 50mV min but on the figure 16, the VBB values shown are linear. Do you use  voltage regulators or  charge pumps to regulate the Back bias voltages?
\end{point}

\begin{reply}
\fix{}{The body bias generator is based on a charge pump circuit. However, the original plot in figure 16 could have been misleading because it reported the optimal BB voltage requested to the controller. We substituted the requested voltage with the 50mV quantized voltage that is practically generated by the BB generators and applied to the wells.}
\end{reply}

%\begin{reply}

%\fix{}{The BB gen has been designed to drive an area of \SI{1}{\milli\metre\squared}. For positive regulation of both wells the BB gen uses a push-pull approach. Negative regulation on the p-well is obtained by means of a dual phase charge pump. Two control loops allow to monitor the impact of the leakage and compensate for wells discharge. The comparators of the feedback use Resistive Digital to Analog Converters (DAC) as references. To reduce the power consumption of the BB gen to \SI{4.5}{\micro \watt}, its operation is duty-cycled, entering a sleep mode where only the leakage is monitored. This paragraph has been integrated in section III, subsection 2.}

%\end{reply}


%push--pull  approach  is used for positive regulation of both wells,  while  a  dual  phase  charge  pump  is  used  to  provide negative regulation on the p-well. A resistive digital  to  analog  converter  generates  the  reference  for comparators, providing the feedback for the two control loops. To reduce power consumption to 4.5 μW, we employ a sleep mode that monitors only the impact of leakage of the wells.

%E' stato progettato per pilorate un'area di 1mm2 (cluster), si è sensibile al leakage, quando le well si scaricano lui le ricarica :), vedi più dettagli nel paper su PULPv3}
\begin{point}
I would like you add all the power consumptions added by this regulation. PMBs, Back Bias generator, thermal sensor,... (i think only the BBG power is written) 
\end{point}
 
\begin{reply}
\fix{}{We did not measure explicitly the power consumption of the PMB circuitry because, by construction, it is not possible to isolate its power consumption contribution from the power consumption of the cluster power domain, being supplied by the same power rail as the rest of the circuit logic. However, we can observe that the PMB subsystem is used for a very short amount of time, which makes its power consumption negligible with respect to the power of the cluster domain on the average.
More specifically, the controller performs a new BB voltage regulation with a frequency of approximately 0.5Hz. During a single BB voltage regulation, the controller reads the PMBs and adjusts the VBB by re-programming the BB generator for a maximum of 16 times or less, if it converges before reaching the last iteration. Every iteration lasts at maximum \SI{4}{\milli \second}, which is the time required to read the output of the PMBs in our configuration. Also, when the PMB circuitry is not used, it is clock-gated. The PMB sub-system is therefore clock-gated for 97\% of the time. Being its area very small compared to the cluster area (less than 0.1\%), we can reasonably assume that the power consumption is negligible if compared to the entire cluster domain power consumption.}
\end{reply}

\begin{point}
Also when you take into account the process and the temperature, do you configure differently the PMBs? or the correction is done only by choosing the correct VBB? Can you explain more accuratly the corrections?
\end{point}

\begin{reply}
\fix{}{The PMBs keep always the same configuration. On the contrary, the linear model that the controller uses to interpret the output of the PMB changes according to the level of knowledge of the operating condition. If the process and the temperature are known, the model accurate, and only small margins are taken on the VBB applied to compensate for PMB measurement error (which is 3\% at 0.7V). If only the temperature is known, the error of the PMB model is higher (4\% at 0.7V), and possible slow process corners are compensated by taking into account wider FBB margins. If both temperature and process corners are unknown, the same principle applies, the uncertainty on the speed of the circuit is further higher (9.7\% at 0.7V), and the controller applies even wider VBB margins to compensate both possible slow process corners and the unknown temperature.}
\end{reply}

\reviewersection
%\textbf{Reviewer 2:}

This paper presents a method to dynamically adjust the body bias of a low-power FD-SOI integrated circuit to the exact performance requirements in order to reduce the leakage current and therefore optimize the power consumption.

It is done using several process monitoring blocks (PMB) consisting of ring oscillators built using cells belonging to the standard cell library used for the design of the circuit. These PMB are characterized for several process corners, voltage supply, and temperature conditions in order to establish correlation laws between the PMB maximum frequency and the chip maximum frequency. An embedded controller partly done by software dynamically regulates the body bias according to the clock frequency requirements in order to minimize the leakage current and therefore the power consumption while guaranteeing that the chip will always be functional at the clock frequency required by the system.

\begin{point}
I found the paper interesting; the proposed method is certainly useful for targeted applications and is clearly explained; the paper presents detailed results useful for the reader.
However, as the Process Monitoring Blocks are done using the standard cell library used for the chip design, it is understandable that they can be representative of the data-path behavior, but not of the memories one. Therefore, it is likely that this method only works when the memories are not part of the critical paths, that is a (potentially acceptable) limitation : for instance, the design could be done in such a way memories are on-purpose put outside the critical paths by adding input and output registers, but this could add latency on memory accesses; could you please introduce a paragraph to discuss this potential issue ? This issue is noted in your introduction for some previous works, but it is not clear for me why it should not apply for this one.
\end{point}

\begin{reply}
\fix{}{In our approach we characterize the relation between the frequency estimated by the PMBs and the maximum frequency of the device independently of where the critical paths are. By deriving a model for the PMBs we embed every mismatch between the frequency predicted by the physical sensors and the actual trend of the maximum frequency versus the VBB in the model itself. Therefore, a potentially unexpected behaviour of the maximum frequency versus the body bias voltage (e.g. given by a critical path going to the memories, or any other unexpected behaviour of the maximum frequency trend) would be embedded in the software model. The advantage of using a software model, rather than relying on fully hardware-based solutions, is that the correlation between the frequency predicted by the sensor and the actual trend of the maximum frequency can be studied afterwards, once the chip is manufactured. By employing the same approach in other digital circuits, an expected difference with respect to the case presented in the paper would be a different model which correlates the output of the sensor and the maximum frequency of the device (e.g. replacing the derived linear model with the resulting PMB model correlating the actual maximum frequency with the PMB prediction).}
\end{reply}


%Therefore, on one side it is true that to safely characterize the output of the PMBs it is important to trigger the critical paths during the maximum frequency estimation. However ,where the most critical paths are is not really relevant for the model parameter extraction because every mismatch would be embedded in the software model}


%\fix{}{3. ---------------------------------- (Avevamo fatto claims sul critical path? avevamo detto dov'era? in questo o altri paper? In general we d don't care, since we can characterize the ratio between the PMB freq and the actual frequency under diferent operating conditions and embed it inti the sw model (e sboriamo dicendo che questo se hai un modello in hardware col cazzo che te lo puoi permettere ;) ) }

\begin{point}
Additionally, I noticed a significant number of typos or details that seem unclear to me and that should be corrected or clarified, as listed below : \\
Page 1 : "Body biasing represents an alternative to adaptation of supply voltage, which is less efficient...": a bit ambiguous : could let think that body biasing is less efficient... \\
Page 2 : Section II: related work, 7th line: "the the" \\
Page 3, column 1, lines 20, 21: "to to" \\
Page 3: Column 2, line 3 : "CPR": not previously defined, or is it CPM ? \\
Page 3: Column 2, lines 17, 18: "fit better" : replace by "better fit" ? \\
Page 3, column 2, Paragraph B, line 2: "the performance have" : either "the performance has", either "the performances have" \\
Page 3, column 2, Paragraph B, line 11: "accordingly to" : according to \\
Page 3, column 2, Paragraph B, line 16: "can not" : cannot \\
Page 4, column 2, paragraph IIIA: "in mplemented" \\
Page 4, column 2, paragraph IIIA: "close the threshold" : close to the threshold \\
Page 5, column 1 : please, define the SCM acronym \\
Page 6, column 2, near the end of the page : "it is reported 1" : reported by (1) \\
Page 7, column 2, paragraph D: "fabricate": fabricated \\
Page 7, column 2, paragraph D: "classified in": classified into \\
\end{point}

\begin{reply}
\fix{}{Typos have been corrected in the text. Thanks for spotting them.}
\end{reply}

\begin{point}
Page 8, figure 9: is there really a 300\% error, or is there a scale mistake ?
\end{point}

\begin{reply}
\fix{}{Yes, it was a scale mistake, it has been fixed it in the figure.}
\end{reply}

\begin{point}
Page 8, column 2: "compensate": compensated

Page 10, column 1: "as we have demonstrated in section": as we have demonstrated it in section
\end{point}

\begin{reply}
\fix{}{Errors have been fixed in the text.}
\end{reply}

\begin{point}
Page 10, column 2: "The only constraint to ensure proper calibration is to execute the procedure at a known temperature": If done at boot-time, how to know the temperature ? Using an on-chip temperature sensor ? how to calibrate the temperature sensor ?
\end{point}

\begin{reply}
\fix{}{"Known temperature" could be misleading with respect to the message that we wanted to convey in this section. We substituted it with "constant temperature". The absolute value of the temperature is not really relevant in this context, and a calibration procedure can be executed even with a non-calibrated temperature sensor, the constraint is that the temperature should remain constant during the calibration procedure to not influence the characterization of the PMB sensor.
Then, starting from a controller calibrated on a constant temperature value, two scenarios are possible:
1. the temperature does not change with respect to the calibration point, and the controller has to compensate with VBB margins the 3\% of model uncertainty at 0.7V (the operating condition reported in Fig. 5).
2. the temperature changes with respect to the calibration point, and the controller has to compensate a slightly higher model uncertainty, which takes into account the effect of temperature change, which is approximately 4\% at 0.7V (the condition reported in Fig. 6).
In both cases, the on chip temperature sensor, even if it is not calibrated to output the true temperature at which the chip is operating, can be safely used.
This explanation has been integrated in section V, subsection A.}
\end{reply}

%\fix{}{The statement "At the boot" is probably misleading, there is not need to execute the procedure at every boot of the system. The only requirements is to establish a correlation between the maximum frequency of the circuit and the PMB output on a set of known temperature points. The proposed calibration procedure can be executed for example when the chip is mounted on a pcb, during its testing, to extract the parameters of the model that will be used by the controller. One aspect which could potentially affect the proper working of the controller is the different aging of the circuit and the PMBs, in that case a re-calibration would extract the new correlation values. The different aging of the circuit and the PMBs is not addressed by this work}

\begin{point}
Page 10, column 2: "either returning wrong arithmetic results of completeley failing": either returning wrong arithmetic results or completly failing"

Page 11, figure 14: Ftarget + Fmax : isn't it Ftraget - Fmax ?
\end{point}

\begin{reply}
\fix{}{Yes, we fixed it in the block diagram. Thanks for spotting the issue.}
\end{reply}

\begin{point}
Page 11, column 2, line 5: "it is been": it is being, or better, it is\\
Page 11, column 2, line 9: "the models compute" : the modes compute\\
Page 11, column 2, line 16: "very close the maximum" : very close to the maximum\\
Page 11, column 2, line 17: "the controller is applying": the controller applies\\
Page 12, column 1, line 6: "the the"\\
Page 12, column 2, legend of figure 17: "this plot whos": this plot shows\\
Page 12, legend of figure 17: below 10°C, is not possible : below 10°C, it is not possible\\
\end{point}

\begin{reply}
\fix{}{Errors have been fixed in the text. Thanks for spotting them.}
\end{reply}

\begin{point}
Page 12, column 2, figure 17: correspondance of curves is unclear: it may be understood that it is better not to take into account process and temperature
\end{point}

\begin{reply}
\fix{}{To clarify ambiguities we rephrased the caption. The red curve reports the leakage current when the controller is off. The green curve shows the Leakage current when the controller is on and the process corner is known. The yellow curve refers to the case where the controller is on but the process corner is not known. In this condition, to guarantee the operating frequency, additional FBB margins are used, resulting in a leakage current increase. Blue curve shows an ideally compensated leakage current, i.e. when no FBB margins are used by the controller.}
\end{reply}


\reviewersection
%\textbf{Reviewer 3:}

\begin{point}
Interesting and well written paper

However, more details on transistor level implementation of the various elements would be more than welcomed, even simple schematics.
\end{point}

\begin{reply}
\fix{}{PMBs and the related circuitry have not been designed by us. These modules have been provided directly by the chip manufacturer (STMicroelectronics) and are protected by a Non Disclosure Agreement.}
\end{reply}

\begin{point}
The procedure for mesuring the Fmax during calibration is well explained, but the choice of the sequence of operation doesn't seem easy. How is it "carefully crafted" ? What level of knowledge of the circuit is needed ?
\end{point}

\begin{reply}
\fix{}{For the benchmark to be effective, it has to trigger the critical paths of the circuit. These paths must be identified during post-layout timing analysis. Also, if the critical path is in the control flow logic of the chip, and not in the data-path, the calibration procedure must be supervised by an external unit (e.g. a microcontroller on the same board) which is capable to reset the chip when it enters irreversible failure states.
We explicitly mentioned the critical path identification during post-layout simulation in section IV, subsection A, footnote 2.}
\end{reply}

\begin{point}
Also, the benchmark includes a mix of arithmetic and memory operations. Nonetheless, SOC and cluster domains have separated back bias, with separated process monitoring circuits. How this double tuning is really handled during operation ? Why only one BBGEN is not sufficient?
\end{point}

\begin{reply}
\fix{}{The two power domains are completely isolated, and the application of a BB voltage on one of them does not affect the other. The reason why there are two body bias generator is to have the possibility to independently apply a BB voltage on each power domain. In this work we focused on performing the compensation with BB only on the cluster power domain, because it is the most computationally capable and power hungry domain; it hosts the 4 cores. On the contrary, the SoC power domain hosts only the peripheral and uDMA subsystem. The same principle presented for the cluster power domain could have been be applied to the SoC power domain.
We integrated this comment in the introduction to clarify that the compensation applies only to one of the two power domains (section I).}
\end{reply}

\begin{point}
Rough evaluation of the time needed for the calibration of BBGEN to obtain Fmax would be nice since it should be made during test time.
\end{point}

\begin{reply}
\fix{}{The duration of a complete calibration depends on the granularity of the sweep performed on both VBB and Fmax, how the maximum frequency is searched (i.e. linear sweep vs binary search), and how long is the executed benchmark. In our example, we used approximately 30 VBB points (1.5V/50mV) and a linear sweep with a 1MHz step. At every evaluation point we executed 10000 benchmark iterations. The overall duration was approximately 6s. 
This comment has been integrated in section V subsection A.}
\end{reply}

\begin{point}
Not enough details for optimizing the control loop are provided, whereas the authors are stated at the same time as critical regarding undershots. Wouldn't limiting overshoot also be beneficial ? Fig 15 seems to exhibit large overshot for example.
Was it tradeoff for good damping of undershots ? Also there is a typo on the y-axis of the first (MHz/ GHz).
\end{point}

\begin{reply}
\fix{}{In this context, overshoots are not critical. During an overshoot, the chip is biased for a short amount of time with more than necessary FBB. Therefore, For a short amount of time, the maximum frequency of the chip is faster than the requested frequency. On the contrary, during undershoots the controller applies less FBB than required (or even RBB). Therefore, the chip is slower than the requested frequency. This condition is critical and very likely determines a chip failure. The reason for the peak resembling an overshoot is not related to the dynamic of the PID but is due to the fact that the controller starts from a fixed zero VBB condition when a new frequency set-point is requested.
This comment has been integrated in section V subsection, C.}
\end{reply}

\begin{point}
The integration of the temperature sensor is not always clear. Included on the chip micrograph, in some measure graphs, but not in the Fig. 14 control loop for example.
\end{point}

\begin{reply}
\fix{}{The knowledge of the exact temperature is not needed for the VBB regulation loop itself reported in Fig. 14. All the temperatures reported for the preliminary characterization of the PMBs in  Fig. 4, Fig. 5, Fig. 6, Tab. IV and Tab V are not measured with the on-chip temperature sensor but externally enforced and regulated on the chip package. Additionally, 
if the chip has been characterized at different temperatures with the procedure reported in Fig. 13, according to the current one at which the system is operating, a different set of model coefficients (e.g. Tab. III for 25 degrees at 0.7V) is used by the controller.
we explicitly mentioned that the temperatures reported in the characterization phase are externally enforced, additionally, we clarified the role of the on-chip temperature sensor in section V, subsection A.}
\end{reply}

\begin{point}
The power consumption gain is stated only at max temperature for one design point. Also, the 1.3x gain stated is not supported by Fig. 18 (only a 15\% reduction can be seen).
\end{point}

\begin{reply}
\fix{}{Yes, the X factor on the energy efficiency changes according to the clock frequency, 1.3X is practically achievable in a typical application scenario, with the system clocked at 150MHz. However the worst case scenario is when the system is clocked with the maximum frequency achievable at 25 degrees, which is approximately 170MHz, and is the one for which the power is reported in the plot. 
We fixed the result to report numbers coherent with Fig. 18.}
\end{reply}

\begin{point}
It is also not clear that the back bias is maintaining frequency for maximum efficiency.
\end{point}

\begin{reply}
\fix{}{We added a sentence to the introduction to explicitly mention that the  aim  of  this  work  is  to  propose  a  performance-aware body  biasing  strategy  to  compensate  for  process  and  temperature  variations  while  guaranteeing  with  minimum  power overhead  a  user-specified  target  frequency.}
\end{reply}

\begin{point}
Graphs would be easier to read with y-x grids, even with a limited number of lines.

Typo at the last sentence of IV. C. "sensors"
\end{point}

\begin{reply}
\fix{}{Errors have been corrected in the plots and text.}
\end{reply}


%}

==> Content/embedded_setup.tex <==
\section{Embedded setup}
Since the final goal of this work is to develop a fully automated body-bias control strategy, the analysis of the PMBs performed on the chip's testing equipment and the proposed methodology have been validated on a real embedded system. More specifically, the applied body bias voltage and the leakage current have been measured on a PULPv3 evaluation. The temperature have been enforced on the chip thanks to a Peltier's element cell regulated by an industrial TEC controller. The entire testing setup is reported in \figurename{ \ref{fig:}}.


==> Content/old-Characterization.tex <==
9\section{Model}
\label{sec:model}

\subsection{Experimental Setup}
\label{sec:setup}

%To compare the ambient temperature and process variations on next generation ULP devices, we conducted a large data acquisition test directly on the PULPv3 prototypes, measuring power and performance metrics at the different corner cases. Based on the measurement results, we have derived a set of empirical models to describe the dependency of the performance metrics to the physical parameters, compensation knobs and environmental conditions. This models will be discussed in the next sections of the paper.

The PMB models derivation, as well as the body bias model described in the following sections are performed with an Advantest SoCV93000 tester system, in connection with a Thermonics 2500E temperature forcing system, able to force an environment temperature ranging from \SI{-80}{\celsius} to \SI{220}{\celsius}. 
Since we are interested in using the body-biasing voltage as independent variable both for temperature and process variations compensation, we structured the measurements as follows: \textit{i)} We defined the operating point (OP) in terms of \{Supply voltage $V_{dd}$ , Temperature\}. More specifically, the voltage corners are: $V_{dd}$ = \{\SI{0.5}{\volt},\SI{0.7}{\volt},\SI{0.9}{\volt}\}. Temperature corners are: T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}; 
\textit{ii)} For each OP we swept the body-biasing voltage ($V_{bb}$) in the range \SI{-1}{\volt} to $V_{dd}/2$ + \SI{300}{\milli \volt} using the body-bias generator.
At every operating point we measured: the leakage power ($P_{LKG}$), the active dynamic power ($P_{DYN}$), the total power ($P_{TOT}$) and maximum frequency ($F_{MAX}$) achievable by the device.
We measured the active dynamic power ($P_{DYN}$) as the difference between the total power ($P_{TOT}$) and the leakage power ($P_{LKG}$).
The total power ($P_{TOT}$) has been measured as the power consumption when the device is executing a benchmark application and the leakage power ($P_{LKG}$) as the power consumption when the device is not clocked. 

We extracted the maximum operating frequency ($F_{MAX}$) by means of a carefully crafted benchmark (i.e. a sequence of arithmetic operations and memory stores), able to trigger the most critical paths\footnote{The critical path has been identified by the timing analysis in the communication between the cores and the scm memory} of the circuit. We verified that the result of the benchmark was returned with the correct timing, and the End-Of-Computation\footnote{Physical output pin of the device which certifies that the system completed all the operations and properly entered a known final state.} signal was properly asserted. 
As cross-check, we verified that the result of the benchmark returned a valid check-sum.

\subsection{PMB characterization}
\label{analysis}

%The first part of the methodology proposed in this paper has the aim to exploit the run-time maximum frequency measurement, performed with the test equipment, to determine the actual maximum frequency of the chip. In parallel, by observing the PMBs' output, it is possible to find a correlation between the actual maximum frequency and the one predicted by the PMBs.
%Once the equation to translate the PMB frequency estimation in $F_{Max}$ has been found, given a target frequency specified by the application and depending on the $V_{dd}$, the body-bias voltage can be finely regulated to fill the performance's gap.

First part of the analysis focuses on the characterization of the performance monitoring blocks placed in the power domain of interest, that is the one hosting the core cluster. The aim of this step is to obtain a model allowing to correlate the response of the frequency probes (PMBs) to the maximum frequency of the device. To obtain the model, we simultaneously measured both the response of the PMBs ($F_{PMB}$) and the maximum chip frequency ($F_{MAX}$) versus the full body bias range. This operation has been repeated per each operating point ($V_{DD}$, $T$). \tablename{ \ref{tab:meas_details}} reports more details regarding the measurement operating conditions.

\begin{table}[htb]
    \centering
    \begin{tabular}{c|c|c|c}
    \toprule
        PULP $V_{DD}$ & $V_{BB}$ & $T_{op}$ & Process corner\\ \midrule
        \SI{0.7}{\volt} & \SI{-1}{\volt} to \SI{650}{\milli \volt} & \SI{25}{\celsius} & Typical \\
    \bottomrule
    \end{tabular}
    \\[5pt]
    \caption{Measurement operating conditions under which the PMB analysis has been performed}
    \label{tab:meas_details}
\end{table}

The aim of this step is to obtain an evaluation of the PMB accuracy. To perform the measurement in a well-defined environment, the temperature is externally enforced and kept constant by the temperature forcing system. The measurements that we performed in this phase are referred to a single chip, this allows to exclude a priori the process variations as possible source of error. Since the entire set of PULPv3 chips have been pre-characterized in terms of maximum performance, we know if the device in exam belongs to a \textit{Fast}, \textit{Typical} or \textit{Slow} process corner. \figurename{ \ref{fig:frequency}} reports the measurement of the $F_{PMB}$ and $F_{MAX}$ versus $V_{BB}$ for a typical device supplied at \SI{0.7}{\volt}.
%For the sake of simplicity, in this section we will not consider the variations introduced by the process; accordingly with this assumption, we assume to use a model calibrated on the specific chip. In other words, the correlation between the value provided by the PMB sensor and the maximum achievable frequency of the chip is calculated for the specific device under test. \figurename{\ref{fig:frequency}} shows on the same plot the maximum frequency measured with the test equipment and the PMB estimation for a typical device at \SI{0.9}{\volt} and \SI{25}{\celsius}

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/FPMB_raw.pdf}
    %\missingfigure[figheight=7cm]{correlation linearity for different chips}
    \caption{This plot compares the maximum achievable frequency and the PMB frequency estimation for a "Typical" PULPv3 chip at \SI{0.7}{\volt} and \SI{25}{\celsius}.}
    \label{fig:frequency}
\end{figure}

%As shown in \figurename{\ref{fig:correlation}}, the relationship between the values provided by the PMB and the maximum frequency of the device can be modeled with a simple affine function\footnote{ The $C_{corr}$ parameter represents the ratio between the delay of the critical paths and the minimum delay determining the frequency of the oscillator inside the PMB. The $F_{0}$ parameter is an offset related to the critical path of the circuit.} (Equation \ref{eq:model}).

In the second phase of the PMB characterization we evaluated the correlation between $F_{PMB}$ and $F_{MAX}$. As shown in  \figurename{ \ref{fig:correlation}}, the model we found is the linear function reported in \ref{eq:model}. In \figurename{ \ref{fig:correlation}} is reported the linear fit of the data.

\begin{equation}
\label{eq:model}
    F_{MAX} = C_{corr} F_{PMB} + F_{0}
\end{equation}

%\tablename{ \ref{tab:model}} shows the parameters of the linear fit at the three OPs for a single device. Notice that the $C_{corr}$ is always lower than 1, which means that the maximum frequency of the circuit is always lower than the the one generated inside the PMBs. The R-Square parameter is always equal or higher than 0.995, indicating that the model properly describes the data's trend.

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{C550925correlation2}
    \caption{This plot shows the correlation between the maximum frequency and the PMB frequency estimation for a typical chip at \SI{0.9}{\volt} and \SI{25}{\celsius}. The data have been fitted with a linear model, the parameters of the fit are: y=mx+q where m=0.6 and q=8.7, R-Square (COD) = 0.995.}
    \label{fig:correlation}
\end{figure}

We repeted the same measurements in different operating corners proving the robustness of the model: \tablename{ \ref{tab:model}} reports the parameters of the model.

\begin{table}[hbt]
    \centering
    \begin{tabular}{l|c|c|c}
    \toprule
        $V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\ \midrule
        $C_{corr}$ & 0.6 & 0.59 & 0.47 \\
        $F_{0}$ & 8.72 & 5.19 & 3.21\\
        R-Square & 0.995& 0.998 & 0.998\\
        \bottomrule
    \end{tabular}
    \\[5pt]
    \caption{Parameters of the model for a typical chip at three different supply voltages and \SI{25}{\celsius}.}
    \label{tab:model}
\end{table}

%The equation we use to correlate the maximum frequency with the PMB frequency estimation, as well as other techniques used in other work, can be affected by errors.
%In our case the error is represented by the residuals of the measurements with respect to the fitting curve. The maximum residual we report for the correlation model, at fixed Operating Point, and for a single device, is the 3\%. Comparable errors are reported also in \cite{Beigne2015}, a similar study performed on a DSP architecture implemented with the same FD-SOI technology and exploiting a performance monitor system based on Timing Fault Sensors (TMFLT).
As a final step for this preliminary PMB characterization we estimated the error of the model, which is represented by the residuals of the measurements with respect to the fitting curve. Table \ref{tab:temp-proc} (\textit{Process-aware Temperature-aware} model) shows the maximum errors we report for the correlation model, for a single device. Comparable errors are reported also in \cite{Beigne2015}, where a similar study performed on a DSP architecture implemented with the same FD-SOI technology, exploiting a performance monitor system based on Timing Fault Sensors (TMFLT).


%The presence of the model's error, that is a frequency uncertainty affecting the Maximum frequency estimation, can be compensated by means of additional forward body-bias. Notice that the $V_{bb}$ margin added to compensate the model's uncertainty, is conceptually different from the $V_{bb}$ regulation to achieve a target frequency. The approach used to compensate the error will be discussed in the next section.

\subsection{Temperature Variations}
\label{temperature}

%The model we propose for the temperature-induced variation compensation is a generalization of the approach we described for a single operating point. To derive a more general fitting function, we performed the same data analysis on the entire data set (multiple OPs) introducing hence an additional degree of freedom. Thanks to this analysis, we obtained a general equation describing all the operating points for a single device. 
%In \figurename{\ref{fig:perchip_model}} is reported the entire set of measurements performed at different voltages and temperatures for a typical device. The red solid line, which is described by the equation \ref{eq:model}, represents the general model fitting the data. Table \ref{tab:model_temp} reports the parameters of the model in this case as well as the R-Square.

Once the robustness of the PMB model has been proved in a given operating condition, it is possible to generalize the analysis to cover a wide temperature operating range. The measurements described in this section are performed on a single chip, supplied with a given voltage ($V_{DD}$), at multiple temperatures. The approach is the same we followed in the previous case, the only difference is that the fitted data are now related to three different temperatures, specifically T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.

\begin{table}[b]
\centering
    %\caption{Model parameters}
    \begin{tabular}{l|c}
    \toprule
        $V_{dd}$ & \SI{0.7}{\volt}\\ \midrule
        $C_{corr}$ & 0.59 \\ 
        $F_{0}$ & 5.42 \\ 
        R-Square & 0.996\\
    \bottomrule
    \end{tabular}
    \\[5pt]
    \caption{Parameters of the model fitting the data for a single chip, at a given supply voltage, at three different temperatures, T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.}
    \label{tab:model_temp}
\end{table}

\figurename{ \ref{fig:perchip_model}} shows the global linear fit. The red solid line, which is described by the equation \ref{eq:model}, represents the general model fitting the data. Table \ref{tab:model_temp} reports the parameters of the model in this operating condition, as well as the R-Square. As in the previous case, we evaluated the error. \figurename{ \ref{fig:perchip_error}} shows the residuals with respect to the fitting curve. As expected, a model which fits data belonging to measurements at various temperatures is affected by a larger error. This phenomenon is caused by the fact that we are assuming that the maximum frequency is limited only by the PMB related to the PMOS transistors, which is usually slower than PMB related to the NMOS ones. Correlation between the maximum frequency of the device and a linear combination of both PMB could improve the accuracy. 



\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{temp_with_bands}
    \caption{In this plot are shown all the measurements performed at a single supply voltage $V_{dd}$ = \SI{0.7}{\volt} and three different temperatures T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}. The red solid line represents the curve  fitting the data measured at the three different temperature.}
    \label{fig:perchip_model}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{error-temp-new}
    \caption{This plot shows the distribution of the relative error versus the maximum frequency when the general model is used to convert the PMB output value in $F_{max}$.}
    \label{fig:perchip_error}
\end{figure}

\subsection{Process variations}
\label{process}

%In this section we generalize the methodology we proposed to reduce the sensitivity to temperature' variations to compensate also process' variations.
Operating temperature is not the only factor affecting device performance operating in near threshold. In this section we will present a short discussion on the performance variance among different chips fabricate in the UTBB FD-SOI technological node caused by different process corners. Then, we will show how the performance monitoring methodology described so far can be further generalized to cover also multiple chips belonging to various process corners. Particular attention should be given to the nature of the performance variation related to the technological process, the variations introduced by the process can be classified in two types: \textit{i)} The Inter-chip variations, that can be observed in terms of performance gaps between different devices, as shown in \figurename{ \ref{fig:frequency_distribution}} \textit{ii)} Intra-chip variations, as demonstrated by \cite{Zandrahimi2016}, resulting in different first N critical path, that can affect the consistency between the behaviour of the circuit and an on-chip performance monitor, confirmed also by our analysis.

%Here, we discuss the results of the analysis performed on a population of 8 different chips. In figure \figurename{\ref{fig:process_model}} are reported the correlation data of all the chips in exam, for a given OP. Notice that the variations introduced by the process can be classified in two types: \textit{i)} The Inter-chip variations, that can be observed in terms of performance gaps between different devices, as shown in \figurename{\ref{fig:frequency_distribution}} \textit{ii)} Intra-chip variations, as demonstrated by \cite{Zandrahimi2016}, resulting in different first N critical path, that can affect the consistency between the behaviour of the circuit and an on-chip performance monitor, confirmed also by our analysis.

\begin{figure}[b]
    \centering
    \includegraphics[width = \columnwidth]{frequency_distribution}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{Normalized distribution of the maximum frequency for the entire population of 48 chips at \SI{0.9}{\volt}, \SI{25}{\celsius}.}
    \label{fig:frequency_distribution}
\end{figure}

As in the case of one chip at multiple temperatures, the model has been obtained by performing a global fit on the data related to chips belonging to different process corners, finding the best function describing them with minimum error. \figurename{ \ref{fig:process_model}} shows the PMB analysis related the chips in exams and the fitting curve.

\begin{figure}[t]
    \centering
    \includegraphics[width = \columnwidth]{fit_temp2.pdf}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{In this plot are represented the data of 3 devices belonging to \textit{Fast}, \textit{Typical} and \textit{Slow} process corners, the dashed line represents the model fitting the data-set}
    \label{fig:process_model}
\end{figure}

It can be noted that also in this case the model is represented by the same linear function \ref{eq:model} shown previously. However, in this case the fitted data have a larger variability, and as a consequence, we observed a larger error and lower R-square. Table \ref{tab:model_temp_process} shows the values of the parameters and the R-Square.
When the chip was fabricated the technology node was at a very early stage, according to \cite{Mackay2006}, the variance introduced by the manufacturing process is expected to decrease with the maturity of the process.

%As for the temperature variation compensation, we derived a general correlation model between all the chips. \figurename{\ref{fig:process_error}} shows the error when this model is used to convert the output of the performance monitor sensor. Also in this case the model is the one described by equation \ref{eq:model}, table \ref{tab:model_temp_process} reports the values of the parameters and the R-Square; notice that in this case the fitted data have a larger variability, resulting in a larger Prediction band and lower R-square.

\begin{table}[htb]
\centering
    \begin{tabular}{l|c}
        \toprule
        $V_{dd}$ & \SI{0.7}{\volt}\\ \midrule
        $C_{corr}$ & 0.614 \\
        $F_{0}$ & 6.86 \\
        R-Square & 0.88\\
        \bottomrule
    \end{tabular}
    \caption{Parameters of the model fitting the data related to chips belonging to different process corners, at a given supply voltage, at three different temperatures.}
    \label{tab:model_temp_process}
\end{table}

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{figuresN/errors}
    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max freq on 10 chips}
    \caption{This plot shows the distribution of the relative error versus the maximum frequency when the process-independent model is used to convert the PMB output value.}
    \label{fig:process_error}
\end{figure}

%To generalize the model and compensate the error, as in the previous section, we derived the function that links the $v_{bb}$ with the relative frequency change at different supply voltages. As shown in figure \figurename{\ref{fig:relative-freq}}, the sensitivity of the frequency with respect to the body-bias, in the forward body bias region, decreases when the supply voltage increases. Starting from this assumption, we can assess that, using a $V_{bb}$ margin to compensate a frequency gap at \SI{0.9}{\volt}, at minimum the same frequency gap will be compensated also for lower supply voltages. More specifically, we can state that the frequency sensitivity to body-bias voltage is always higher than 10\%/\SI{100}{\milli \volt}. Using this more general model, as expected, we obtained higher frequency errors (\figurename{\ref{fig:process_error}}).

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width = \columnwidth]{relative-freq-allV}
%    %\missingfigure[figheight=7cm]{study of the correlation between PMBs and max %freq on 10 chips}
%    \caption{The graph shows the Relative frequency sensitivity to the $V_{bb}$ at %different operating points.}
%    \label{fig:relative-freq}
%\end{figure}

\subsection{Body-Bias Model}
The final goal of this study is to develop a performance-aware body bias regulation system. To this end, it is necessary to derive a model which links a variation of the $V_{BB}$ to the $F_{max}$ variation. Once the relationship between these two parameters has been obtained, given a performance gap to be compensate, it is possible to determine the necessary amount of body bias voltage to do it.

\begin{figure}[htb]
    \centering
    \includegraphics[width = \columnwidth]{freq_to_vbb07}
    \caption{This plot shows the relation between the maximum frequency of a typical device and the body-bias voltage at three operating points: Vdd = \SI{0.7}{\volt} and T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.}
    \label{fig:freqvbb}
\end{figure}

It is very important to note that the use of body-bias for this application is twofold: \textit{i)} in an ideal case, that is assuming no errors on the $F_{max}$ estimation, $V_{BB}$ represents the knob to simply change the performance of the device \textit{ii)} in a context where $F_{max}$ is affected by uncertainty because of the reasons previously described, $V_{BB}$ margins can be used to compensate $F_{max}$ negative residuals; in other words, all those conditions where the $F_{max}$ is overestimated by the model. \figurename{\ref{fig:freqvbb}} shows the relationship between $F_{max}$ and $V_{BB}$ at different temperatures.
%Starting from the error estimation, since we assume to know the supply voltage at every OP, we used the empirical model that links the frequency and the body-bias voltage to convert the frequency error in a forward body-bias margin to add to the $V_{bb}$ regulation. Notice that we are interested in aligning the maximum frequency achievable by the chip to the target one, therefore we need to compensate only for negative frequency errors. 
%In other words, we will compensate those conditions where the general model overestimates the real performance of the device.

Despite the curve shifts with temperature, if we consider the relative frequency variation, we can simplify the body bias model approximating the curve with a linear function having $5\%/\SI{100}{\milli \volt}$ (at 0.7V) as slope (\figurename{ \ref{fig:freqvar}}).
Table \ref{tab:perf_gain} shows the same analysis at different voltage operating points.

\begin{table}[tb]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
        PULP \SI{0.5}{\volt} & \SI{0.7}{\volt} & \SI{0.9}{\volt}\\ \midrule
        $11\%/\SI{100}{\milli \volt}$ & $5\%/\SI{100}{\milli \volt}$& $3\%/\SI{100}{\milli \volt}$ \\
        \bottomrule
    \end{tabular}
    \\[5pt]
    \caption{Body bias induced performance gain}
    \label{tab:perf_gain}
\end{table}
%As shown in \figurename{\ref{fig:freqvbb}}, the relationship between the frequency and the body-bias voltage shifts with the temperature, however, as shown by the plot in \figurename{\ref{fig:freqvar}}, once the supply voltage has been fixed, the relative frequency variation (in the forward body-bias region) can be considered in first approximation as temperature-independent; because the three curves are superimposed.

\begin{figure}[tb]
    \centering
    \includegraphics[width = \columnwidth]{frequency-variation}
    \caption{In this plot is represented the relative frequency variation versus the body-bias voltage, with respect to the $V_{bb}$ = \SI{0}{\volt} condition. The operating points are: Vdd = \SI{0.7}{\volt} and T = \{\SI{-20}{\celsius},\SI{25}{\celsius},\SI{80}{\celsius}\}.}
    \label{fig:freqvar}
\end{figure}

This model allows to compute the additional body bias margin required to compensate the measurement errors described in the previous sections. Assuming to compensate the model uncertainty caused by temperature, which was the 3\% at \SI{0.7}{\volt}, we need to add a margin on $V_{BB}$ of \SI{75}{\milli \volt}.

It can be noted that body bias margins can be summed as independent contributions, to compensate different errors of the models. Assume to use a model which has several uncorrelated error sources: 3\% intrinsic error (PMB sensor), 1\% originated by temperature variations and 5.7\% generated by process variations. The resulting 9.7\% total error can be compensated with the sum of the body bias margins that would separately compensate each error\cite{Kumar2008a}.
As a concluding remark for this section, it can be noted that to minimize the error of the model, a calibration procedure capable to discover the chip process corner is required. This calibration procedure reduces the error by a factor of 2.4 and is described in section \ref{sec:controller}.
%Starting from this assumption, the amount of additional forward body bias that allows to neglect the effects of temperature variation can be calculated exploiting the relative frequency versus body-bias voltage relation reported in \figurename{\ref{fig:freqvar}}, which is the frequency-normalized inverse of \figurename{\ref{fig:freqvbb}}. To give an example, assuming that we want to compensate the error at \SI{0.9}{\volt} shown in \figurename{\ref{fig:perchip_error}}, that is the 3\% in the worst case, we need to consider a $V_{bb}$ margin of \SI{0.1}{\volt} (The amount of body-bias is derived by the curves in \figurename{\ref{fig:freqvar}}). Notice that the additional amount of $V_{bb}$ causes an increase in the leakage current, hence additional leakage power consumption; the overhead caused by this methodology will be discussed in section \ref{sec:overhead}.




%As anticipated in the previous section, we considered the variations introduced by the process and the variations introduced by the temperature as separated. As demonstrated in \cite{Kumar2008a}, the additional body-bias voltage used to reach the target frequency, plus the margin to compensate the uncertainty of the model, can be summed to the fraction of $V_{bb}$ used to compensate process' variations as independent contributions.


\subsection{Methodology Overhead}
\label{sec:overhead}

%The methodology we propose uses the forward body-biasing to compensate the uncertainties in process monitor readings. Since the $V_{bb}$ has a straightforward effect on the leakage current, hence on the leakage power consumption, it is important to quantify the overhead introduced by the body-bias margins. As it is well known, the higher is the frequency of the system, the more dominant is the dynamic power consumption with respect to the leakage power. Hence, the overhead decreases as the target frequency increases, since only the leakage power changes when the FBB is applied.
%Notice that we define the overhead as the additional leakage power with respect to the global power consumption, assuming to calculate it in the most common operating condition for a near-threshold processor, that is when the system is running at the maximum achievable frequency, given a supply voltage.

The compensation methodology we propose is based on the application of forward body bias to compensate process and temperature variations. As it is well known, FBB has a direct influence on the leakage current of a circuit, hence it is important to quantify the overhead associated with the additional body bias margins. Specifically, we defined the overhead as the ratio between the additional leakage caused by the body bias margin and the leakage current of the circuit when an ideal controller is regulating the body bias voltage (i.e. capable to apply the exact $V_{BB}$ to achieve a given target frequency). How the additional leakage current affects the global power consumption strongly depends on the dynamic power consumption (i.e operating frequency) of the circuit, hence the overhead will be computed with respect to the leakage current under the \textit{ideal} body bias regulation.

%The following tables report the worst case overheads at three different conditions: \textit{i)} when the Process-unaware model is used \textit{ii)} when it is possible to calibrate the model on the single chip \textit{iii)} when we can fully characterize the operating point knowing also the temperature.

The overhead presented in this section refers to the three different models derived in the previous sections. More specifically, to the cases where the supply voltage is known and \textit{i)} the process corner and the temperature are unknown, we define this model as \textit{Process-Unaware Temperature-Unaware model} \textit{ii)} the process corner is known and the temperature is unknown, we refer to it as \textit{Process-Aware Temperature-Unaware model} \textit{iii)} both temperature and process corner are known, which is the \textit{Process-Aware Temperature-Aware model}.

When the \textit{Process-Unaware Temperature-Unaware} model is used, we experience the highest overhead. As expected, the higher is the uncertainty of the model, the wider is the body bias safety margin required to use the model, and also the higher is the associated overhead because of the higher leakage current. However, having the possibility to determine the chip process corner and calibrate the model on the specific device (i.e. passing to the \textit{Process-Aware Temperature-Unaware } model) the overhead can be significantly reduced. If we consider the leakage current associated with the body bias margins needed to correct the errors of the \textit{Process-Aware Temperature-Unaware} model, we can observe that the overhead is much lower. Finally, probing also the temperature, it would be possible to use multiple, better correlated, \textit{Process-Aware Temperature-Aware} PMB models at different temperatures. Table \ref{tab:temp-proc} summarizes the results in terms of overhead.

\begin{table}[hbt]
    \centering
    \begin{tabular}{l|c|c|c}
    \toprule
        $V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\
        
    \midrule
        \multicolumn{4}{l}{Proc-unaware/Temp-unaware \hfill}\\
    \midrule
        $F_{err}$ & 6.6\% & 9.7\% & 25\% \\
        $V_{BB}$ margin [mV] & 150 &  150& 200\\
        Leakage overhead & 33\% & 37\% & 66\%\\
    \midrule
        \multicolumn{4}{l}{Proc-aware/Temp-unaware}\\
    \midrule
        %$V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\
        $F_{err}$ & 3\% & 4\% & 7\% \\
        $V_{BB}$ margin [mV]& 100& 100& 100\\
        Leakage overhead & 13\% & 14\% & 15\%\\
    \midrule
        \multicolumn{4}{l}{Proc-aware/Temp-aware}\\
    \midrule
        %$V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\
        $F_{err}$ & 2\% & 3\% & 6\% \\
        $V_{BB} $ margin [mV] & 50& 50& 50\\
        Leakage overhead & 9\% & 10\% & 12\%\\
   \bottomrule
    \end{tabular}
    \\[5pt]
    \caption{Frequency error of the three presented models and power consumption overheads with respect to the ideal compensation where no body bias margins are used.}
    \label{tab:temp-proc}
\end{table}

%Assuming to probe also the temperature, the only error affecting the model is the one given by the fitting curve, which is the 5\% in the worst case (\SI{0.5}{\volt}), resulting in a worst case overhead of the 3\%.

%In the first case, the worst case model error to compensate with additional body bias margin is the 5\% ($V_{DD} = \SI{0.5}{\volt}$), that is the biggest residual between the measurements and the curve fitting the data of a single chip at a single temperature. We measured that the additional leakage caused by the body bias margin added to correct such error represents the 3\% of the global power consumption.


%When the model can be calibrated on the specific device, it is possible to reduce the error in the maximum frequency estimation approximately of a factor of 3. Table \ref{tab:temp} shows the results in terms of frequency errors and overhead in this condition.
%\begin{table}[hbt]
%    \centering
%    \begin{tabular}{r|c|c|c}
%        $V_{dd}$ & \SI{0.9}{\volt} & \SI{0.7}{\volt} & \SI{0.5}{\volt}\\
%        $F_{err}$ & 3\% & 4\% & 7\% \\
%        Leakage overhead & 13\% & 14\% & 15\%\\
%    \end{tabular}
%    \caption{Frequency error and power consumption overhead for temperature effect compensation.}
%    \label{tab:temp}
%\end{table}

%When only the supply voltage is known, it is necessary to compensate temperature and process variations, as a consequence, the frequency error in the estimation of the maximum one is high and also the power consumption overhead. Table \ref{tab:temp-proc} summarize the results at three different operating voltages.




            %\figurename{\ref{fig:overhead}} shows the trend of the overhead for different supply voltages, when the temperature is equal to \SI{80}{\celsius}, hence when the influence of the leakage on the dynamic power is maximum.
            
            % \begin{figure}[htb]
            %     \centering
            %     \includegraphics[width = \columnwidth]{overhead_temp}
            %     %\missingfigure[figheight=7cm]{overhead}
            %     \caption{Worst case overhead caused by the temperature effect compensation at three different operating points: $V_{dd}$ = \{\SI{0.9}{\volt} , \SI{0.7}{\volt} , \SI{0.5}{\volt}\}.}
            %     \label{fig:overhead}
            % \end{figure}
            
            % Concerning the overhead to compensate process variations, it can be calculated as an additional contribution to the temperature compensation's overhead. \figurename{\ref{fig:overhead_gen}} shows the global overhead versus the target frequency 
            
            % \begin{figure}[htb]
            %     \centering
            %     \includegraphics[width = \columnwidth]{global_overhead}
            %     %\missingfigure[figheight=7cm]{overhead}
            %     \caption{Worst case overhead including the compensation of both the temperature and process variations.}
            %     \label{fig:overhead_gen}
            % \end{figure}






